A State Sum Model for (2+1) Lorentzian Quantum Gravity

A state sum model based on the group SU(1,1) is defined. Investigations of its geometry and asymptotics suggest it is a good candidate for modelling (2+1) Lorentzian quantum gravity.

==> Geom/geoquant.tex <==
\section{Quantum Vectors}\label{quant-vect}

It is known in the case of the compact group $SU\left(2\right)$ that
there is an intimate relationship between its unitary representations
and `quantum vectors' in $\R^3$.  One can construct this relationship
in roughly the following way.  For any Lie group, $G$, there is a
natural action on its Lie algebra $\mathfrak{g}$, called the adjoint
representation, given by
$$
g\circ u = g u g^{-1}
$$
and of the Lie algebra on itself
given by the Lie bracket
\begin{equation}
u\stackrel{v}{\longmapsto}v\left(u\right) = \comm{v}{u}
\end{equation}
for $u,v\in\mathfrak{g}$, $g\in G$.

In the case of the Lie algebras $\su{2}$ and $\su{1,1}$ there is a
invariant bilinear form, given by the standard trace in
the fundamental representation, that defines a pairing between the Lie
algebra and its dual. In this case there are natural actions of both
the group $G$ and the Lie algebra $\mathfrak{g}$ on
$\mathfrak{g}^\star$ called the coadjoint representation 

For $f\in\mathfrak{g}^\star$ define the action of $g\in G$ as
$$
f\longmapsto g\circ f
$$
with 
\begin{equation}
\ip{g\circ f}{v} = \ip{f}{g^{-1}\circ v} = \ip{f}{g^{-1} v g}
\end{equation}
similarly the action of $u\in\mathfrak{g}$ on $\mathfrak{g}^\star$ is
defined as
$$
f  \longmapsto u\circ f
$$
where $u\circ f\in\mathfrak{g}^\star$ is defined via its natural
pairing with the Lie algebra by
\begin{equation}
\left(u\circ f\right)\left(v\right) = f\left(\comm{u}{v}\right)
\end{equation}
both for arbitrary $v\in\mathfrak{g}$

Now if $G$ acts on a vector $f\in\mathfrak{g}^\star$ the set of fixed
points under the group action is denoted $G_f$ and its Lie algebra
$\mathfrak{g}_f$. The coadjoint orbit of $f$ under $G$,
$\mathcal{O}_f$, is identified with the quotient space $G/G_f$ and is
a smooth manifold.  The coadjoint representation has a natural
symplectic structure on its orbits given as follows.

Let $b\in\mathfrak{g}^\star$, the
coadjoint orbit $G\circ b$ is the orbit of $b$ under the action of the
whole Lie group, the symplectic form, $\omega$  satisfies
$$
\omega: T G\circ b\times T G\circ b\longrightarrow\C
$$ 
where $T G\circ b$ is the tangent space to the coadjoint orbit.

Now $SU\left(2\right)$ as a manifold is the 3-sphere, $S^3$, and its
tangent space (Lie algebra) is naturally identified with $\R^3$,
equipped with the standard Euclidean metric as discussed in section
\ref{rep}.  The existence of the metric allows the tangent and
cotangent spaces to be identified and the group structure then defines
an action on $\R^3$, in the co-adjoint representation, by
rotations, since $SU\left(2\right)$ is the double cover of
$SO\left(3\right)$.  The orbits of cotangent vectors $v\in\R^3$ then
define the coadjoint orbits and are 2-spheres since the action of
$SO\left(3\right)$ preserves Euclidean length.

One then wishes to quantise these Euclidean vectors in $\R^3$ by
assigning Hilbert spaces to represent the possible states of each
vector and operators on those Hilbert spaces to the observables.  For
the case under consideration there will be a Hilbert space for each
vector of a given length and then for each such vector the observables
will be simply the components in the $x$, $y$ and $z$ directions.

For the case of $SU\left(2\right)$ the operators that project on each
axis are simply the generators of the Lie algebra $\su{2}$ $J_x$,
$J_y$ and $J_z$.  Thus the problem is reduced to constructing a
unitary representation of $\su{2}$ on certain Hilbert spaces that
correspond to vectors of certain lengths.  Since each vector $v$ is
naturally associated to a coadjoint orbit, $\Omega_v$, and since a
coadjoint orbit has a natural symplectic manifold, being two
dimensional and inheriting a natural volume form, one may construct
such a series of Hilbert spaces by the method of geometric
quantisation\cite{Wood}.

Roughly speaking the Hilbert space, $\mathcal{H}_v$, associated to
each vector $v$ is constructed as the space of square integrable
sections of a line bundle $\Gamma^\omega$ over the coadjoint orbit
$\Omega_v$.  Then each observable $f\in\C^\infty\left(\Omega_v\right)$
corresponds to an operator, $\delta_f$, on $\mathcal{H}_v$ via
\begin{equation}
\delta_s\left(s\right) = -i\hbar\nabla^\omega_{X_f}s+fs
\end{equation}
where $s\in\mathcal{H}_v = L^2\left(\Gamma^\omega\right)$,
$\nabla^\omega_X$ is the connection compatible with the hermitian
structure on $L^2\left(\Gamma^\omega\right)$ whose curvature is
precisely $\frac{\omega}{i\hbar}$ with $\omega$ the symplectic form
that defines the volume form on the coadjoint orbit. For the
$SU\left(2\right)$ case since the coadjoint orbits are two dimensional
the volume form simply is the symplectic form.

The vector field $X_f$ is defined, again using the symplectic form
via,
$$
\omega\left(X_f,\bullet\right) = -df\left(\bullet\right)
$$
The Hilbert space, $L^2\left(\Gamma^\omega\right)$, of square
integrable sections has inner product given by, for $s,t\in
L^2\left(\Gamma^\omega\right)$,
$$
\ip{s}{t} = \int_{\Omega} \left(s,t\right)_x\, \omega
$$
where for each point $x\in\Omega$ the inner product on the fibre is
determined by a local trivialisation of the section.  That is if
$l_1,l_2\in \pi^{-1}\left(x\right)$ with $\pi:\Gamma\to\Omega$ the
projection onto the base space then there is a local trivialisation
over $x\in\Omega$ given by
$$
\psi\left(l_i\right) = \left(x,z_i\right)
$$
for $z_i\in\C$ and the inner product is simply defined as
multiplication of complex numbers via
$$
\left(l_1,l_2\right)_x = \bar{z_1}z_2
$$

This construction is what is meant by a `quantisation' of a classical
mechanical system. Here, typically, the symplectic manifold would
arise as the phase space of some mechanical system for which a
quantisation was being sort.   

The key question is thus when is this construction of a complex line
bundle and connection compatible with the symplectic form possible so
as to allow a quantisation of a given system.  It turns out\cite{Wood}
that it is possible in a globally consistent way to construct such a
line bundle if the symplectic form defines an integral cohomology
class for the symplectic manifold.  This integrality condition
requires
\begin{equation}
\frac{1}{h}\int_{\Omega}\omega\in\Z
\end{equation}
with $h$ Planck's constant.

For $SU\left(2\right)$ the symplectic form, $\omega$, on its coadjoint
orbits is given by the natural volume form on the sphere of radius $R$,
namely $\omega = R\sin\theta\,d\theta\wedge d\phi$. The integrality
condition thus requires
$$
\frac{1}{h}\int_0^\pi\int_0^{2\pi}R\sin\theta\,d\theta d\phi \in\Z
$$
or that $\frac{4\pi R}{h}\in\Z$.  Thus quantisation is only possible
for the spheres of radius $j\hbar$ with $2j\in\N$ and the length of
the vector has become quantised in units of $\frac{\hbar}{2}$.  One
may then proceed to construct the action of the generators of \su{2}
on the square integrable sections and recover the finite dimensional
unitary representations of \su{2}\cite{Flude} and the unitary
representations determine the quantum geometry of 3-dimensional
Euclidean vectors.

\bigskip

\subsection{The Discrete Series}

For $SU\left(1,1\right)$ the coadjoint orbits are more involved than
$SU\left(2\right)$.  The Lie algebra \su{1,1} is naturally identified
with $\R^3$ again, but this time with an indefinite Lorentzian metric,
by virtue of $SU\left(1,1\right)$ being the double cover of the
3-dimensional Lorentz group $SO\left(2,1\right)$ as discussed in
section \ref{rep}.  The coadjoint orbits are then the orbits of
certain Lorentzian vectors, $v$, under the action of
$SO\left(2,1\right)$.

The Lie algebra \su{1,1} is given by the following traceless 
hermitian matrices
\begin{equation}\label{su11-lie}
K_1 = \frac{1}{2}\left(\begin{array}{cc}
0 & 1\\ 1 & 0
\end{array}\right),\;\;
K_2 = \frac{1}{2}\left(\begin{array}{cc}
0 & i\\ -i & 0
\end{array}\right),\;\;
K_3 = \frac{1}{2}\left(\begin{array}{cc}
1 & 0\\ 0 & -1
\end{array}\right)
\end{equation}


Now consider the vector $\pm\lambda f_3\in\mathfrak{g}^\star$ dual to
the $K_3$, that is $\ip{f_3}{K_i} = \delta_{3,i}$.  The set of fixed
points $G_{\pm\lambda f_3}$ is the $g\in G$ such that $K_3 = g^{-1} K_3
g$, or
\begin{equation}
G_{\pm\lambda f_3} = \left(\begin{array}{ccc} e^{i\phi} & 0\\0 & e^{-i\phi}
\end{array}\right)
\end{equation}
for $\phi\in\left[0,2\pi\right]$.  The fact that $f_3$ is left
invariant by the $SO\left(2\right)$ group of space like rotations imply
it is geometrically a time like vector in $\R^3$, which for convenience
is taken as future pointing.

Now, to construct the coadjoint orbit associated to this
time like vector $\pm\lambda f_3$ decompose the a group element in
the following way. For $g\in G$, as in section \ref{rep}, 
$$
g = \left(\begin{array}{cc}
\alpha & \beta\\ \bar{\beta} & \bar{\alpha}
\end{array}\right)
$$
let $z = \frac{\beta}{\bar{\alpha}}\in\C$ and choosing
$\phi\in\left[0,2\pi\right]$ so that $\alpha = \frac{e^{i\phi}}
{\sqrt{1-z\bar{z}}}$ and $\beta = \frac{e^{i\phi}
z}{\sqrt{1-z\bar{z}}}$ one may write\cite{Ba47}
$$
g = \frac{1}{\sqrt{1-\left|z\right|^2}}\left(\begin{array}{cc}
1 & z\\\bar{z} & 1
\end{array}\right)
\left(\begin{array}{cc}
e^{i\phi} & 0\\ 0 & e^{-i\phi}
\end{array}\right)
$$
In this parametrisation the Haar measure on $G$ becomes
$\Lambda\frac{d\phi dz d\bar{z}}{\left(1-\left|z\right|^2\right)^2}$,
for some constant $\Lambda$.  It is now a simple matter to construct
the space $G/G_{\pm\lambda f_3}$; it is parameterised by a single
complex variable $z$ with $\left|z\right| < 1$ and is thus the
Poincar$\acute{\mathrm{e}}$ disk. The volume measure descends as the
symplectic form $\omega = i\Lambda\frac{ dz\wedge
d\bar{z}}{\left(1-\left|z\right|^2\right)^2}$ for some constant $\Lambda$.

Now the space $\left(G/G_{\pm\lambda f_3},\omega\right)$ is Kahler and
one may choose a polarisation in which either $z$ or $\bar{z}$ is
covariantly constant as both are preserved by the group action. The
first choice leads to an action on holomorphic functions on $D$, while
the second gives an action on anti-holomorphic functions.

It remains to construct the representation of the group $G$ on the
space of $L^2$ functions in $z$ alone. $g\in G$ acts on $f\in
L^2\left(G\right)$ via
$$
\left(g\circ f\right)\left(h\right) = f\left(h g\right)
$$
for $h\in G$.  This then induces an action on $L^2$ functions on the
Poincar$\acute{\mathrm{e}}$ disk, $D$, which respects the
polarisation, indeed one finds the action on the quotient space
$G/G_{\pm\lambda f_3}$ is given by
\begin{equation}
\left(\begin{array}{cc}
1 & z\\ \bar{z} & 1
\end{array}\right)\longmapsto
\left(\begin{array}{cc}
1 & \frac{\beta + \bar{\alpha}z}{\alpha + \bar{\beta}z}\\
\frac{\bar{\beta} + \alpha\bar{z}}{\bar{\alpha} + \beta\bar{z}} & 1
\end{array}\right)
\end{equation}
which implies an action of $G$ on holomorphic functions in
$L^2\left(D\right)$ by fractional linear transformations
\begin{equation}\label{G-on-D}
\left(g\circ f\right)\left(z\right) = 
f\left(\frac{\beta + \bar{\alpha}z}{\alpha + \bar{\beta}z}\right)
\end{equation}

Now the norm on $L^2\left(D\right)$ is given by using the standard
symplectic form $\omega$ to integrate the norm on the fibres over the
base space
\begin{equation}\label{disc-metric}
\ip{f}{g} = \int \ip{f}{g}_z i\Lambda\frac{ dz
d\bar{z}}{\left(1-\left|z\right|^2\right)^2}
\end{equation}
Taking the norm on each fibre as 
\begin{equation}\label{fibre-metric-1}
\ip{f}{g}_z = \bar{f}\left(z\right)g\left(z\right)
\end{equation}
it is clear there are no holomorphic functions $f$ with
$\left|f\right|^2 < \infty$.  One therefore looks for a deformation
of equation \ref{fibre-metric-1} so 
\begin{equation}\label{fibre-metric}
\ip{f}{g}_z = \xi\left(z\right)\bar{f}\left(z\right)g\left(z\right)
\end{equation}
where the function $\xi$ falls off sufficiently fast at the disk's
boundary to allow $L^2$ functions to exist.

Now, one wishes to think of the new inner product in equation
\ref{fibre-metric} as the same inner product as equation \ref{fibre-metric-1}
with the sections $f$ and $g$ multiplied by the real function
$\xi^{\frac{1}{2}}\left(z\right)$.  The curvature, $\Omega$, defined 
in local coordinates, $x^i$, by
$$
\Omega\left(\frac{\partial}{\partial x^i},
\frac{\partial}{\partial x^j}\right) = 
\frac{i}{2}\left(
\nabla_{\frac{\partial}{\partial x^i}}
\nabla_{\frac{\partial}{\partial x^j}} - 
\nabla_{\frac{\partial}{\partial x^j}}
\nabla_{\frac{\partial}{\partial x^i}}
\right)
$$
transforms as
\begin{equation}
\Omega = i
\frac{\partial^2}{\partial\bar{z}\partial z} \left(\xi\right)^{\frac{1}{2}} 
dz\wedge d\bar{z}
+ \Omega_0
\left(\xi\right)^{\frac{1}{2}} 
\end{equation}
where $\Omega_0$ is the curvature 2-form for the original metric in
equation
\ref{fibre-metric-1}.  Choosing this to be zero and requiring that the
curvature of the connection be the symplectic 2-form $\omega$ implies
$\xi$ is determined by
\begin{equation}
\frac{\partial^2}{\partial\bar{z}\partial z} \chi
 = \frac{\Lambda}{\left(1-z\bar{z}\right)^2}
\end{equation}
where $\xi^{\frac{1}{2}} = \exp\left\{\chi\right\}$.  Solving this
then gives
$$
\xi = \left(1-z\bar{z}\right)^{-2\Lambda}
$$
Now the inner product on sections over $D$ is given by
\begin{equation}
\ip{f}{g} = \int \bar{f}\left(z\right)g\left(z\right)
\left(1-z\bar{z}\right)^{-2\Lambda-2}\Lambda\,dzd\bar{z}
\end{equation}
but the action of the group on $D$, given by equation \ref{G-on-D}, no
longer preserves it.  To restore an invariant measure on the quotient
space functions on $D$ must now transform under the action of the
group as
\begin{equation}\label{pos-act}
f\left(z\right)\longmapsto\left(\alpha +
\bar{\beta}z\right)^{2\Lambda} f\left(\frac{\beta +
\bar{\alpha}z}{\alpha + \bar{\beta}z}\right)
\end{equation}
For this action to be single valued one evidently requires
$2\Lambda\in\Z$.

Now a basis for holomorphic functions on $D$ is given by the monomials
$\left\{1,z,z^2,z^3,\dots\right\}$ and $L^2\left(D\right)$ is non
empty when
\begin{equation}
\int\left(1-z\bar{z}\right)^{-2\Lambda-2}\Lambda\,dzd\bar{z}
<\infty
\end{equation}
or $\Lambda\le -1$.  Thus one has precisely recovered the action of
the positive discrete series by geometrically quantising a future
pointing time like vector.

The anti-holomorphic polarisation leads to functions in $\bar{z}$
alone while the transformation under the action of the group given by
equation \ref{pos-act} is unchanged.  Alternatively one may regard it
again as functions in $z$ alone which transform as
\begin{equation}
f\left(z\right)\longmapsto\left(\alpha +
\bar{\beta}\bar{z}\right)^{2\Lambda} f\left(\frac{\beta +
\bar{\alpha} z}{\alpha + \bar{\beta}z}\right)
\end{equation}
under the action of the group. This is then precisely the action of
the negative discrete series.





It is of note that the discreteness of the discrete series does not
arise from an integrality condition ($\omega$ is topologically
trivial) but from requiring the group to act in a single valued way.

\subsection{The Continuous Series}

Now consider the vector given by $\lambda f_1$, the dual vector to
$K_1$ in equation \ref{su11-lie}.  The set of fixed points $G_{\lambda
f_1}$ are $g\in G$ such that $K_1 = g^{-1} K_1 g$ or
$$
G_{\lambda f_1} = \pm\left(\begin{array}{cc}
\cosh\chi & \sinh\chi\\ \sinh\chi & \cosh\chi
\end{array}\right)
$$
This time, since the vector is invariant under an $SO\left(1,1\right)$
subgroup, it is a space like vector being dealt with.  The quotient
space $G/G_{\lambda f_1}$ may be exhibited most easily in the setting of
$SL_2\left(\R\right)$. A generic element of this group may be
decomposed as
\begin{equation}\label{sl2r-decomp}
\begin{pmatrix}
a & b\\ c & d
\end{pmatrix} = 
\begin{pmatrix}
1 & \xi\\ 0 & 1
\end{pmatrix}
\begin{pmatrix}
1 & 0\\ \psi & 1
\end{pmatrix}
\begin{pmatrix}
e^{\chi} & 0\\ 0 & e^{-\chi}
\end{pmatrix}
\end{equation}
for real numbers $\psi$, $\xi$ and $\chi$ with $ad-bc=1$. A plus sign
is chosen if $d > 0$, and if $d < 0$ then a minus sign is chosen so
that equation \ref{sl2r-decomp} covers the whole of
$SL_2\left(\R\right)$ except where $d = 0$.

The $SO\left(1,1\right)$ subgroup of fixed points is now realised as
the matrix
$$
\pm\begin{pmatrix}
e^{\chi} & 0\\ 0 & e^{-\chi}
\end{pmatrix}
$$

$G$ then acts on the quotient space from the right as
\begin{multline}\label{gquant-b}
\left(\begin{array}{cc}
1 & \xi\\ 0 & 1
\end{array}\right)
\left(\begin{array}{cc}
1 & 0\\ \psi & 1
\end{array}\right)
\longmapsto
\left(\begin{array}{cc}
1 & \frac{a\xi+c}{b\xi+d}\\ 0 & 1
\end{array}\right)
\left(\begin{array}{cc}
1 & 0\\ \psi +\frac{b}{b\xi+d} & 1
\end{array}\right)
\left(\begin{array}{cc}
b\xi+d & 0\\ 0 & \frac{1}{b\xi+d}
\end{array}\right)\\
\equiv\pm\mathrm{sign}\left(b\xi+d\right)\left(\begin{array}{cc}
1 & \frac{a\xi+c}{b\xi+d}\\ 0 & 1
\end{array}\right)
\left(\begin{array}{cc}
1 & 0\\ \psi +\frac{b}{b\xi+d} & 1
\end{array}\right)
\end{multline}





Chooses a polarisation in which $\psi$ is covariantly constant. This
is then clearly preserved by the action of the group (which is linear
in $\psi$) so the reduced Hilbert space is simply
$L^2\left(\R\right)$, or square integrable functions in $\xi$ alone.

The volume form transforms as
$d\xi\mapsto\frac{d\xi}{\left(b\xi+d\right)^2}$ so an invariant inner
product is given by
\begin{equation}
\ip{f}{g} = \int_{-\infty}^\infty
\bar{f}\left(\xi\right)g\left(\xi\right) d\xi
\end{equation}
with $f\in L^2\left(\R\right)$ transforming under the action of $G$ as
\begin{equation}\label{contin}
\left(g\circ f\right)\left(\xi\right)
= \epsilon^\pm\left(b\xi+d\right)
\left|b\xi+d\right|^{is-1} f\left(\frac{a\xi+c}{b\xi+d}\right)
\end{equation}
for arbitrary $s\in\R$ so that the action of $G$ preserves the norm of
each function where the symbol $\epsilon^\pm\left(a\right)$ is defined
as
\begin{align*}
\epsilon^+\left(a\right) & = 1\\
\epsilon^-\left(a\right) & = \mathrm{sign}\left(a\right)
\end{align*}

Equation \ref{contin} is simply the standard action of
$SL_2\left(\R\right)$ in the continuous series; thus the geometric
quantisation of a space like vector is simply the continuous series of
representations.




==> Racah/racahdis-simple.tex <==

\section{The Racah Coefficients for the Discrete Series} \label{rac}

In this section explicit calculations will be made for the case where
all the representations are in the discrete series.  In contrast to
section \ref{CGC} the Clebsch-Gordon coefficients will be exhibited in
the $SO\left(2\right)$ discrete basis since the calculations are
easier in this form and the Racah coefficient is basis independent as
discussed in section \ref{Racah}.

We shall start with two lemmas that will be of use later

\begin{lem} \label{lem1}
\begin{multline}
\frac{\G{a+1}}{\G{b+1}\G{c+1}} =\\ \sum_n
\frac{\G{a-b+1}\G{a-c+1}}
{\G{a-b-n+1}\G{a-c-n+1}\G{b+c-a+n-1}\G{n+1}}
\end{multline}
\end{lem}

Lemma \ref{lem1} follows from the addition theorem for binomial
coefficients by expanding both sides of $(a+b)^n (a+b)^m =
(a+b)^{n+m}$ and equating powers of $a$ and $b$ as in \cite{RacahI}.

One also has the following for $n\in\Z^+$
\begin{multline*}
\frac{\G{a+n}}{\G{a}} = \left(a+n-1\right)\left(a+n-2\right)\dots
\left(a+1\right) a\\
= \left(-1\right)^n\left(1-a-n\right)\left(2-a-n\right)\dots
\left(-a-1\right)\left(-a\right)
= \left(-1\right)^n\frac{\G{1-a}}{\G{1-a-n}}
\end{multline*}
so that the following analytic continuation for $\Gamma$
functions holds
\begin{lem}\label{lem2}
$$
\frac{\G{a+n}}{\G{a}} = \left(-1\right)^n\frac{\G{1-a}}{\G{1-a-n}}
$$
for $n\in\Z^+$, $a\in\C$, $a\not\in\Z$
\end{lem}
as a consequence to lemma \ref{lem2} the following holds
\begin{equation}\label{an-cont}
\frac{\G{a}\G{1-a}}{\G{b}\G{1-b}} = \left(-1\right)^{a-b}
\end{equation}
for $a,b\in\Z^+$.  To see this note that from \ref{lem2} one has for
$k\in\C$, $k\not\in\Z$.
$$
\frac{\G{a+k}\G{1-a-k}}{\G{b+k}\G{1-b-k}}
= \frac{\G{k}\G{1-k}}{\G{k}\G{1-k}}\left(-1\right)^{a-b}
= \left(-1\right)^{a-b}
$$
now let $k\to 0$ and since the right hand side is independent of $k$
one may remove the requirement $k\not\in\Z$ and the equation becomes
equation \ref{an-cont}.

Finally there is the Gauss summation formula\cite{HypGeo}
\begin{lem}\label{lem3}
$$
\sum_{n}\frac{\G{a+n}\G{b+n}\G{c}}{\G{a}\G{b}\G{c+n}\G{n+1}}
= \frac{\G{c}\G{c-a-b}}{\G{c-a}\G{c-b}}
$$
\end{lem}

From section \ref{rep} the positive discrete series is characterised
by the following action of the generators of \su{1,1} on the Hilbert
spaces $\mathcal{H}_j$ with basis $\{\ket{j,m} |\;
j,m\in\frac{1}{2}\N,\;\; m\ge j\}$
\begin{align*}
K_3\ket{j,m} & = m\ket{j,m}\\
K_\pm\ket{j,m} & = \pm\sqrt{(m\pm j)(m\mp j\pm 1)}\ket{j,m\pm 1}
\end{align*}
while the negative discrete series simply has $m\mapsto -m$.

The Clebsch-Gordon coefficients for the discrete series may be defined
as follows
\begin{equation}\label{CGC-def-O2}
\ket{j\left(j_1 j_2\right),m} = \sum_{m_1,m_2} \left[
\begin{array}{ccc} j_1 & j_2 & j\\ m_1 & m_2 & m \end{array} \right]
\ket{j_1,m_1}\otimes\ket{j_2,m_2}
\end{equation}
with $m = m_1 + m_2$.  An explicit formula for the Clebsch-Gordon
coefficient may be derived via a recursion relation in the manner of
Holman and Biedenharn's approach to the problem (see for instance
\cite{HoBi66} and \cite{HoBi68}). Their formula for the Clebsch-Gordon 
coefficient of coupling in the discrete series consists of the two
solutions $\left[\begin{array}{ccc} j_1 & j_2 & j
\\ m_1 & m_2 & m\end{array}\right]_+$ and 
$\left[\begin{array}{ccc} j_1 & j_2 & j
\\ m_1 & m_2 & m\end{array}\right]_-$ where
\begin{multline}\label{cg}
\left[\begin{array}{ccc} j_1 & j_2 & j
\\ m_1 & m_2 & m\end{array}\right]_+ = 
\delta_{m_1+m_2,m}\\ \times
\sqrt{\frac{\G{m-j+1}\G{m+j}\G{m_1-j_1+1}\G{j_1-j_2+j}\G{j_1+j_2+j-1}}
{\G{m_2-j_2+1}\G{j_2+m_2}\G{m_1+j_1}\G{-j_1+j_2+j}\G{-j_1-j_2+j+1}}}\\
\times\HypT{j_2+m_2}{-m_1+j_1}{m_2-j_2+1}{m_2-j-j_1+1}{m_2+j+j_1}{1}
\end{multline}
and
\begin{equation}\label{cg2}
\left[\begin{array}{ccc} j_1 & j_2 & j
\\ m_1 & m_2 & m\end{array}\right]_- = 
\left[\begin{array}{ccc} j_2 & j_1 & j
\\ -m_2 & -m_1 & -m\end{array}\right]_+
\end{equation}
The particular solution used depends on the case of coupling.

Here a slightly different normalisation to Holman and Beidenharn's
original formula is being used so that the specific formula satisfies
the orthonormality relations in equations \ref{CGC-orth} and
\ref{CGC-orth2},  specifically the usual factor of $\sqrt{2j-1}$ has
been omitted.  Note also that Holman and Beidenharn's formula has the
$j$'s as negative half integers, whereas in equation \ref{cg}
the $j$'s are the more usual positive half integers.

The generalised hypergeometric function\cite{HypGeo} is defined
via
$$
\HypT{a}{b}{c}{d}{e}{z}
= \sum_n \frac{\G{a+n}\G{b+n}\G{c+n}\G{d}\G{e}z^n}
{\G{a}\G{b}\G{c}\G{d+n}\G{e+n}\G{n+1}}
$$
and converges if $-a-b-c+d+e > 0$.


The discrete basis version of the recoupling identity in equation
\ref{racah} may be expressed as
\begin{multline}\label{racah-discrete}
\sum_{m_{12}} 
\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
m_1 & m_2 & m_{12} \end{array} \right]
\left[ \begin{array}{ccc} j_{12} & j_3 & j\\ 
m_{12} & m_3 & m \end{array} \right]\\
= \sum_{j_{23}\;m_{23}} (2j_{23}+1) 
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ j_3 & j & j_{23} 
\end{array}\right\}
\left[ \begin{array}{ccc} j_2 & j_3 & j_{23}\\
m_2 & m_3 & m_{23} \end{array} \right]
\left[ \begin{array}{ccc} j_1 & j_{23} & j\\ 
m_1 & m_{23} & m \end{array} \right]
\end{multline}
where $\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\  m_1 & m_2 &
m_{12} \end{array} \right]$ are the Clebsch-Gordon coefficients for
the coupling of two unitary irreducible representations of $SU(1,1)$. 

The discrete basis version of the orthonormality relations in equation
\ref{CGC-orth} now becomes
\begin{equation}
\sum_{m_1}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ m_1 & m-m_1 & m \end{array} \right]
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ m_1 & m-m_1 & m \end{array} \right]
 = \frac{1}{2j-1} 
\end{equation}
and this relation may be used to bring equation \ref{racah-discrete}
into the following form
\begin{multline} \label{racdef}
\sum_\beta\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
m_1 & \beta & m_1 +\beta \end{array} \right]
\left[ \begin{array}{ccc} j_{12} & j_3 & j\\ 
m_1 +\beta & j_{23}-\beta & j_{23} + m_1 \end{array} \right]
\left[ \begin{array}{ccc} j_2 & j_3 & j_{23}\\ 
\beta & j_{23}-\beta & j_{23} \end{array} \right]\\
= \left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
j_3 & j & j_{23} \end{array}\right\}
\left[ \begin{array}{ccc} j_1 & j_{23} & j\\ 
m_1 & j_{23} & m_1 + j_{23} \end{array} \right]
\end{multline}
where the choice $m_{23} = j_{23}$ has been made.

Depending on the case of coupling one then uses either of
$
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_\pm
$.  From \cite{HoBi68} one must
take
$$
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right] = 
\begin{cases}\renewcommand{\arraystretch}{0.7}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_+ & 
\text{ for }j_1,j_2,j_{12}\in\mathcal{D}^+\\
\renewcommand{\arraystretch}{0.7}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_- & 
\text{\parbox{5cm}{ for $j_1,j\in\mathcal{D}^+$, 
$j_2\in\mathcal{D}^-$\\[-3.5mm] $\,m \ge j_1-j_2$, $m>0$}}\\
\renewcommand{\arraystretch}{0.7}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_+ &
\text{\parbox{5cm}{ for $j_1\in\mathcal{D}^+$,
$j_2,j\in\mathcal{D}^-$\\[-3.5mm] $m \le j_1-j_2$, $m<0$}}\\
\renewcommand{\arraystretch}{0.7}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_- & 
\text{ for }j_1,j_2,j_{12}\in\mathcal{D}^- 
\end{cases}
$$

Now consider the representations $j_1$, $j_2$ and $j_3$.  Formally
there are $2^3 = 8$ different combinations of positive and negative
discrete representations, however these come in dual pairs so there
are only four unique possibilities.  It is now a simply matter to
enumerate the possibilities for the remaining discrete series
representations in the Racah coefficent in table \ref{posneg-racah}.

\begin{table}[hbt!]
\begin{center}
\begin{tabular}{ccccccc}
Case & $j_1$ & $j_2$ & $j_3$ & $j_{12}$ & $j_{23}$ & $j$\\
(1) & + & + & + & + & + & +\\
(2) &$-$& + & + & + & + & +\\
(3) &$-$& + & + &$-$& + & +\\
(4) &$-$& + & + &$-$& + &$-$\\
(5) & + & + &$-$& + & + & +\\
(6) & + & + &$-$& + &$-$&$-$\\
(7) & + & + &$-$& + &$-$& +\\
(8) &$-$& + &$-$& + & + & +\\
(9) &$-$& + &$-$& + & + &$-$\\
(10)&$-$& + &$-$&$-$& + &$-$\\
(11)&$-$& + &$-$& + &$-$&$-$\\
(12)&$-$& + &$-$&$-$&$-$&$-$\\
\end{tabular}
\end{center}
\caption{The possible unique distributions of positive and negative discrete 
representations in the Racah coefficient\label{posneg-racah}}
\end{table}

It now remains to calculate the Racah cofficient for the twelve cases
given in table \ref{posneg-racah}.  Let the Racah coefficient for each
of the twelve cases of coupling be denoted by a subscript $N$ for
$N=1\dots 12$.  Explicitly the calculation for cases 1 proceeds from a
substitution of equation
\ref{cg} into \ref{racdef}, where equation \ref{racdef} has been written
\begin{multline} 
\sum_\beta\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
j-j_{23} & \beta & j-j_{23} +\beta \end{array} \right]
\left[ \begin{array}{ccc} j_{12} & j_3 & j\\ 
j-j_{23} +\beta & j_{23}-\beta & j \end{array} \right]
\left[ \begin{array}{ccc} j_2 & j_3 & j_{23}\\ 
\beta & j_{23}-\beta & j_{23} \end{array} \right]\\
= \left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
j_3 & j & j_{23} \end{array}\right\}
\left[ \begin{array}{ccc} j_1 & j_{23} & j\\ 
j-j_{23} & j_{23} & j \end{array} \right]
\end{multline}
and the additional choice $m_1 = j-j_{23}$ has been made.  This
allows three of the four Clebsch-Gordon coefficients to be immediately
summed so the Racah coefficient may be written
\begin{equation} \label{rac2}
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ j_3 & j & j_{23} \end{array} 
\right\}_1 = \Delta\left(j_2 j_3 j_{23}\right)
\Delta\left(j_{12}j_3 j\right)\Delta\left(j_1 j_{23} j\right)
\Delta\left(j_1 j_2 j_{12}\right)\,\mathcal{I}
\end{equation}
where
\begin{multline*}
\mathcal{I} =\sum_{t\,\beta}
\frac{\left(-1\right)^{j-j_{23}-j_{12}-j_2+t+2\beta}
\G{\beta+j_2+t}\G{\beta-j_2+1+t}}
{\G{j_{23}-\beta-j_3+1}\G{j_3+j_{23}-\beta}\G{\beta-j_2+1}}\\
\times\frac{1}{\G{j_1+j-j_{23}}\G{\beta-j_{12}+j_1+1+t}\G{j_1+j_{12}+\beta+t}
\G{\beta+j_2}\G{t+1}}\\
\times\frac{1}{\G{1-j_1+j-j_{23}-t}\G{j_2-j_1+j_{12}}\G{j_{12}-j_1-j_2+1}
\G{j+j_{23}-j_1}}\\ \times\frac{1}{\G{j_1+j_{23}+j-1}}
\end{multline*}

$\mathcal{I}$ may be reduced to a single summation as follows.
Introduce a new summation using lemma \ref{lem1} with $a =
\beta-j_2+t$, $b = \beta-j_{12}+j_1+t$ and $c = \beta+j_1+j_{12}+t-1$,
then $\mathcal{I}$ may be written (after an application of equation
\ref{an-cont})
\begin{multline*}
\mathcal{I} = \sum_{\beta\,u\,t}
\frac{\left(-1\right)^{2\beta+j-j_2-j_{12}-j_{23}}
\G{\beta+j_2+t}\G{j_1-j+j_{23}+t}\G{-j_1-j_2-j_{12}+2}}
{\G{j_{23}-\beta-j_3+1}\G{j_3+j_{23}-\beta}\G{\beta-j_2+1}\G{\beta+j_2}}\\
\times\frac{1}{\G{j_1+j-j_{23}}\G{t+1}\G{j_2-j_1+j_{12}}\G{j+j_{23}-j_1}
\G{j_1+j+j_{23}-1}}\\
\times\frac{1}{\G{j_{12}-j_2-j_1-u+1}\G{2-j_1-j_2-j_{12}-u}
\G{2j_1+\beta+j_2+t+u}\G{u+1}}\\
\times\frac{1}{\G{j_1+j_{23}-j}\G{j-j_1-j_{23}+1}}
\end{multline*}

The sum over $t$ is simply a hypergeometric function at $z=1$.  This
may be summed by Gauss' theorem, as in lemma \ref{lem3} with $a =
\beta+j_2$, $b = j_1+j_{23}-j$ and $c = \beta +2j_1+j_2+u$.  The
remaining sums may be written
\begin{multline*}
\mathcal{I} =
\sum_{\beta\,u}\left(-1\right)^{2\beta-j_2+j-j_{23}-j_{12}}
\frac{\G{2-j_2-j_1-j_{12}}\G{j+j_1-j_{23}+u}}
{\G{j_{23}-j_3-\beta+1}\G{j_3+j_{23}-\beta}\G{\beta-j_2+1}}\\
\times\frac{1}{\G{j+j_1-j_{23}}\G{j_2-j_1+j_{12}}\G{j_{23}+j-j_1}
\G{j_1+j_{23}+j-1}}\\\times\frac{1}
{\G{j_{12}-j_1-j_2-u+1}\G{2-j_1-j_2-j_{12}-u}\G{u+1}\G{j-j_1-j_{23}+1}}
\\ \times\frac{1}{\G{2j_1+u}\G{j_1+j_2+j-j_{23}+u+\beta}}
\end{multline*}

Now set $\beta = z+j_2$, with $z$ now guaranteed to be an integer.
The sum over $z$, after two applications of equation \ref{an-cont},
may again be recognised as a hypergeometric function which is
summable by Gauss' theorem, using lemma \ref{lem3} with $a =
j_2+j_3-j_{23}$, $b = 1+j_2-j_3-j_{23}$ and $c = 2j_2+j_1+u+j-j_{23}$.

The final sum over $u$ is a generalised hypergeometric function of
type ${ }_4F_3$ and the sum $\mathcal{I}$ may be written

\begin{multline*}
\mathcal{I} = \left(-1\right)^{j_2+j-j_{23}-j_{12}}
\frac{1}{\G{j_{12}-j_1+j_2}\G{j+j_{23}-j_1}\G{j-j_1-j_{23}+1}}\\
\times\frac{1}{\G{j_{23}-j_2-j_3+1}\G{j_{23}+j_3-j_2}\G{j_{12}-j_1-j_2+1}}\\
\times\frac{1}{\G{2j_1}\G{j_1+j_2+j-j_3}\G{j_1+j_2-1+j_3}}\\
\times\HypF{j_1+j-j_{23}}{j_1+j+j_{23}-1}{j_1+j_2-j_{12}}
{j_1+j_2+j_{12}-1}{2j_1}{j_1+j_2+j-j_3}{j_1+j_2+j_3+j-1}{1}
\end{multline*}

where the generalised hypergeometric function\cite{HypGeo} is defined as
\begin{multline*}
\HypF{a}{b}{c}{d}{e}{f}{g}{z} = \\
\sum_n\frac{\G{a+n}\G{b+n}\G{c+n}\G{d+n}\G{e}\G{f}\G{g}}
{\G{a}\G{b}\G{c}\G{d}\G{e+n}\G{f+n}\G{g+n}\G{n+1}}z^n
\end{multline*}

subsitituting this back into equation \ref{rac2} the final result is
gained
\begin{multline}\label{RacahSU11}
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ j_3 & j & j_{23} \end{array} 
\right\}_1 = \frac{\left(-1\right)^{j_2+j-j_{23}-j_{12}}
\Delta\left(j_2 j_3 j_{23}\right)
\Delta\left(j_{12}j_3 j\right)\Delta\left(j_1 j_{23} j\right)}
{\G{j_{12}-j_1+j_2}\G{j+j_{23}-j_1}\G{j-j_1-j_{23}+1}}\\
\times\frac{\Delta\left(j_1 j_2 j_{12}\right)}
{\G{j_{23}-j_2-j_3+1}\G{j_{23}+j_3-j_2}\G{j_{12}-j_1-j_2+1}}\\
\times\frac{1}{\G{2j_1}\G{j_1+j_2-j_3+j}\G{j_1+j_2-1+j_3}}\\
\times\HypF{j_1+j-j_{23}}{j_1+j+j_{23}-1}{j_1+j_2-j_{12}}
{j_1+j_2+j_{12}-1}{2j_1}{j_1+j_2+j-j_3}{j_1+j_2+j_3+j-1}{1}
\end{multline}


In a similar way one may derive the formula for case 5 from equation
\ref{racdef} again with the choice $m_1 = j-j_{23}$.  Here one has
$$
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}
\\ j_3 & j & j_{23} \end{array} \right\}_5 
= \Delta\left(j_1 j_2 j_{12}\right)
\Delta\left(j_3 j_{23}j_2\right)
\Delta\left(j_{23} j_1 j\right)
\Delta\left(j j_3 j_{12}\right)\mathcal{I}
$$
where, after some rearrangement with equation \ref{an-cont}
\begin{multline}\label{mid5}
\mathcal{I} = \sum_{\beta\,t}
\frac{\left(-1\right)^{t-j+j_3-j_{12}+\frac{1}{2}}
\G{\beta+j_2+t}\G{\beta-j_2+1+t}\G{\beta-j_3-j_{23}+1}}
{\G{j_1+j-j_{23}}\G{\beta+j_1-j_{12}+1+t}\G{\beta+j_1+j_{12}+t}}\\
\times\frac{\G{\beta+j_3-j_{23}}}
{\G{t+1}\G{j_{12}+j_2-j_1}\G{j_{12}-j_1-j_2+1}\G{j_{23}+j-j_1}
\G{j_1+j+j_{23}-1}}\\ \times\frac{1}
{\G{j_2-j_3+1-j_{23}}\G{j_3+j_{12}-j}\G{j_{12}-j-j_3+1}\G{\beta-j_2+1}}\\
\times\frac{1}{\G{\beta+j_2}\G{j_2+j_3-j_{23}}\G{j-j_1-j_{23}-1-t}}
\end{multline}

This may be evaluated by using lemma \ref{lem1}, with $a = \beta
-j_2+t$, $b = \beta-j_{12}+j_1+t$ and $c = \beta+j_{12}+j_1 +t-1$ to
introduce an extra sum, so that equation \ref{mid5} may be written
\begin{multline}
\mathcal{I} = \sum_{\beta\,t\,u}
\frac{\left(-1\right)^{-j+j_3-j_{12}+u+\frac{1}{2}}
\G{\beta+j_2+t}\G{\beta-j_{23}-j_3+1}\G{\beta+j_3-j_{23}}}
{\G{j_1+j-j_{23}}\G{t+1}\G{j_{12}+j_2-j_1}\G{j+j_{23}-j_1}
\G{j_1+j+j_{23}-1}}\\ \times 
\frac{\G{j_{12}+j_1+j_2+u-1}\G{j_{23}+j_1-j+t}}
{\G{j_2-j_3-j_{23}+1}\G{j_{12}+j_3-j}\G{j_{12}-j_3-j+1}\G{\beta-j_2+1}
\G{\beta+j_2}}\\ \times\frac{1}{\G{-j_{23}+j_2+j_3}
\G{j_{12}-j_1-j_2-u+1}\G{\beta+2j_1+j_2+t+u}\G{u+1}}\\
\times\frac{1}{\G{j_{12}+j_1+j_2-1}\G{j_1+j_{23}-j}\G{j-j_{23}-j_1+1}}
\end{multline}

The sum over $t$ is again summable with the Gauss summation formula of
lemma \ref{lem3} with $a = \beta+j_2$, $b = j_{23}+j_1-j$ and
$ c = \beta+2j_1+j_2+u$.  Hence one has

\begin{multline*}
\mathcal{I} = \sum_{\beta\,u}
\frac{\left(-1\right)^{-j+j_3-j_{12}+u+\frac{1}{2}}
\G{\beta-j_3-j_{23}+1}\G{\beta+j_3-j_{23}}\G{j+j_1-j_{23}+u}}
{\G{j_1-j_{23}+j}\G{j_2-j_1+j_{12}}\G{j+j_{23}-j_1}\G{j_1+j+j_{23}-1}}\\
\times\frac{\G{j_1+j_2+j_{12}-1+u}}{\G{j_2-j_3-j_{23}+1}\G{j_{12}+j_3-j}
\G{j_{12}-j-j_3+1}\G{\beta-j_2+1}\G{j_2+j_3-j_{23}}}\\
\times\frac{1}{\G{j_{12}-j_1-j_2-u+1}\G{u+1}\G{j_1+j_2+j_{12}-1}
\G{j-j_1-j_{23}+1}\G{2j_1+u}}\\ \times \frac{1}
{\G{\beta+j_1+j_2+j-j_{23}+u}}
\end{multline*}

As before set $\beta = z+j_2$, with $z$ now guaranteed to be an
integer.  The sum over $z$, after an application of equation
\ref{an-cont}, is a hypergeometric function
which is again summable by Gauss' theorem, using lemma \ref{lem3} with
$a = j_2+j_3-j_{23}$, $b = 1+j_2-j_3-j_{23}$ and $c =
2j_2+j_1+u+j-j_{23}$.

The final sum over $u$ is a generalised hypergeometric function of
type ${ }_4F_3$ and the sum $\mathcal{I}$ may be written
\begin{multline*}
\mathcal{I} = \left(-1\right)^{-j+j_3-j_{12}+\frac{1}{2}}
\frac{1}{\G{j_{12}-j_1+j_2}\G{j+j_{23}-j_1}\G{-j+j_3+j_{12}}}\\
\times\frac{1}{\G{j_{12}-j_3-j}\G{j-j_{23}-j_1+1}\G{j_{12}-j_1-j_2+1}}\\
\times\frac{1}{\G{2j_1}\G{j_1+j_2-j_3+j}\G{j_1+j_2-1+j_3}}\\
\times\HypF{j_1+j-j_{23}}{j_1+j+j_{23}-1}{j_1+j_2-j_{12}}
{j_1+j_2+j_{12}-1}{2j_1}{j_1+j_2+j-j_3}{j_1+j_2+j_3+j-1}{1}
\end{multline*}

The final result is thus
\begin{multline}\label{su11-5}
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}
\\ j_3 & j & j_{23} \end{array} \right\}_5 
= \frac{\left(-1\right)^{-j+j_3-j_{12}+\frac{1}{2}}
\Delta\left(j_1 j_2 j_{12}\right)\Delta\left(j_3 j_{23}j_2\right)}
{\G{j_{12}-j_1+j_2}\G{j+j_{23}-j_1}\G{-j+j_3+j_{12}}}\\
\times\frac{\Delta\left(j_{23} j_1 j\right)
\Delta\left(j j_3 j_{12}\right)}
{\G{j_{12}-j_3-j}\G{j-j_{23}-j_1+1}\G{j_{12}-j_1-j_2+1}}\\
\times\frac{1}{\G{2j_1}\G{j_1+j_2-j_3+j}\G{j_1+j_2-1+j_3}}\\
\times\HypF{j_1+j-j_{23}}{j_1+j+j_{23}-1}{j_1+j_2-j_{12}}
{j_1+j_2+j_{12}-1}{2j_1}{j_1+j_2+j-j_3}{j_1+j_2+j_3+j-1}{1}
\end{multline}

The similarity with the form for the Racah coefficient for case 1 is
not accidental.  Indeed one finds

\begin{multline}
\frac{\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}
\\ j_3 & j & j_{23} \end{array} \right\}_1 }
{\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}
\\ j_3 & j & j_{23} \end{array} \right\}_5 }=
\left(-1\right)^{j_2-2j-j_{23}-j_3-\frac{1}{2}} 
\sqrt{\frac{\G{j+j_3-j_{12}}\G{j-j_3-j_{12}+1}}
{\G{j_{23}-j_2-j_3}\G{j_{23}+j_3-j_2}}}\\ \times
\sqrt{\frac{\G{j_{12}+j_3-j}\G{j_{12}-j-j_3+1}}
{\G{j_2+j_3-j_{23}}\G{j_2-j_3-j_{23}+1}}} 
= \left(-1\right)^{-j+j_3-j_{12}-\frac{1}{2}} 
\end{multline}
with the final equality from suitable applications of equation
\ref{an-cont}.  Thus the two cases are simple analytic continuations,
up to phase, of the same generalised hypergeometric function to
domains where the various labels $j$ satisfy different inequalities.


Finally case 11 will be explicitly computed from equation
\ref{racdef}, this time with the choice $m_1 = -j+j_{23}$ as
$\mathcal{J}_1$ is in the negative discrete series.  Here one has
$$
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}
\\ j_3 & j & j_{23} \end{array} \right\}_{11} 
= \Delta\left(j_1 j_{12} j_{2}\right)
\Delta\left(j_2 j_{23}j_3\right)
\Delta\left(j_{23} j_1 j\right)
\Delta\left(j j_{12} j_{3}\right)\mathcal{I}
$$
where, after some rearrangement with equation \ref{an-cont}
\begin{multline}\label{mid11}
\mathcal{I} = \sum_{\beta\,t}\frac{\left(-1\right)^{t-j_3-j_{23}-j_1+j_{12}}
\G{j_3-j_{23}-\beta}\G{j_{23}+j_{12}-j+\beta}}
{\G{j_3+j_{23}-j_2}\G{j_3+j-j_{12}}\G{j_{23}+j_2-j_{12}-j+1+t}}\\
\times\frac{\G{j_1+j_{23}-j+t}\G{\beta-j_2+1}\G{j_{23}-j-j_1+t+1}}
{\G{j_2+j_{12}+j_{23}-j+t}\G{\beta-t+j_2+1}\G{t+1}
\G{j_{12}+j-j_{23}-\beta}}\\
\times\frac{1}{\G{j+j_{12}-j_{23}-\beta}
\G{j_{12}-j-j_3+1}\G{j_3+j_{12}-j}\G{j_2-j_3-j_{23}+1}}\\ 
\times\frac{1}{\G{j_2+j_3-j_{23}}
\G{j+j_{23}-j_1}\G{j_1+j+j_{23}-1}\G{j_3-j_2-j_{23}+1}}\\
\times\frac{1}
{\G{j_3-j_{12}-j+1}\G{j_{23}+j_3+\beta}}
\end{multline}

As for the previous two cases, this may be evaluated by using lemma
\ref{lem1}, with $a = -\beta +j_2+t-1$, $b = j_{23}+j_2-j-j_{12}+t$ 
and $c = j_2+j_{12}+j_{23}-j+t-1$, to introduce an extra sum, so that
equation \ref{mid5} may be written
\begin{multline}
\mathcal{I} = \sum_{\beta\,t\,s}
\frac{\left(-1\right)^{j_3-j_2-j_1}
\G{j_3-j_{23}-\beta}}
{\G{t+1}\G{j_{12}+j_3-j}}\\
\times\frac{\G{\beta-j_2+1}}
{\G{j_2+j_3-j_{23}}\G{j+j_{23}-j_1}\G{j+j_1+j_{23}-1}
\G{j_3-j_2-j_{23}+1}}\\
\times\frac{1}{\G{j_3+j_{23}+\beta}
\G{j+j_{12}-j_{23}-\beta-s}}\\ 
\times\frac{1}{\G{2j_{23}-2j+j_2+t+\beta+s+1}
\G{s+1}\G{j-j_1-j_{23}-t+1}}\\
\frac{1}{\G{j+j_1-j_{23}-t}\G{j-j_{23}-j_{12}-\beta-s+1}}
\end{multline}

The sum over $t$ may now be recognised as a hypergeometric function
and summed by lemma \ref{lem1} with $a=j_2+\beta+s+1$, $b =
j_1+j_2+j_{23}-j+\beta+s+1$ and $c = j_2+j_{23}-j_1-j+\beta+s+2$.  The
remaining sums may be written
\begin{multline}
\mathcal{I} = \sum_{\beta\,s}
\frac{\left(-1\right)^{j_3+j_{12}+j_{23}-j_1-1}
\G{j_3-j_{23}-\beta}\G{\beta-j_2+1}\G{j_2+\beta+s}}
{\G{j_3+j_{12}-j}\G{j_2+j_3-j_{23}}\G{j+j_{23}-j_1}}\\
\times\frac{1}{\G{j_1+j+j_{23}-1}\G{j_3-j_2-j_{23}+1}
\G{j+j_1-j_{23}}\G{j_3-j-j_{12}+1}}\\
\times\frac{1}{\G{j_3+j_{23}+\beta}\G{j+j_{12}-j_{23}-\beta-s}
\G{j-j_{23}-j_{12}-\beta-s+1}\G{s+1}}\\
\times\frac{1}{\G{j-j_1-j_{23}+1}\G{j_2+j_{23}-j-j_1+\beta+s+1}
\G{j_2+j_{23}-j+j_1+\beta+s}}
\end{multline}

Now introduce two new variables, $z$ and $p$, that satisfy $s =
q-\beta$ and $\beta = p+j_3-j_{23}$.  The sum over $p$ is immediate
from lemma \ref{lem3} with $a = j_3-j_{23}-j_2+1$, $b = j_3-j_{23}-q$
and $c = 2j_3$.  This leaves one remaining sum over $q$ and setting $q
= n+j-j_{23}-j_2+j_1$ this is immediately recognised as an ${ }_4F_3$
generalised hypergeometric function.  Substitution back into equation
\ref{rac2} yields the final result 
\begin{multline}\label{su11-11}
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}
\\ j_3 & j & j_{23} \end{array} \right\}_11 
= \frac{\left(-1\right)^{j_{12}-j_{23}-j-j_2}
\Delta\left(j_1 j_{12} j_{2}\right)
\Delta\left(j_2 j_{23}j_3\right)}
{\G{j_3+j_{12}-j}\G{j_2+j_3-j_{23}}j+j_{23}-j_1}\\
\times\frac{\Delta\left(j_{23} j_1 j\right)
\Delta\left(j j_{12} j_{3}\right)}
{\G{j_3-j_{12}-j+1}\G{j-j_{23}-j_1+1}\G{j_2+j_3+j_{23}-1}}\\
\times\frac{\G{j_2+j_3-j_1-1}}
{\G{2j_1}\G{j_2+j_{12}-j_1}\G{j_2-j_1-j_{12}}\G{j_1+j+j_3-j_2}}\\
\times\HypF{j_1+j-j_{23}}{j_1+j+j_{23}-1}{j_1-j_2+j_{12}}
{j_1-j_2-j_{12}+1}{2j_1}{j_1-j_2+j+j_3}{j_1-j_2-j_3+j+1}{1}
\end{multline}



There are two symmetries one may apply to equation \ref{racdef} in
order to generate the twelve different cases of coupling.

Firstly, consider the symmetry where $j_{12}$ is swapped with $j_{23}$
and $j_1$ is swapped with $j_3$, applied to equation
\ref{racdef}.  One now has
\begin{multline}
\sum_\beta\left[ \begin{array}{ccc} j_3 & j_2 & j_{23}\\ 
j-j_{12} & \beta & j-j_{12} +\beta \end{array} \right]
\left[ \begin{array}{ccc} j_{23} & j_1 & j\\ 
j-j_{12} +\beta & j_{12}-\beta & j \end{array} \right]
\left[ \begin{array}{ccc} j_2 & j_1 & j_{12}\\ 
\beta & j_{12}-\beta & j_{12} \end{array} \right]\\
= \left\{ \begin{array}{ccc} j_3 & j_2 & j_{23}\\ 
j_1 & j & j_{12} \end{array}\right\}
\left[ \begin{array}{ccc} j_3 & j_{12} & j\\ 
j-j_{12} & j_{12} & j \end{array} \right]
\end{multline}

This equation is the defining relation for a Racah coefficient with a
potentially different distribution of positive and negative discrete
series.  In particular it is easy to see from table \ref{posneg-racah}
that it causes the following exchanges: case 2 is swapped with case 5,
case 3 is swapped with case 7, case 4 is swapped with case 6 and case
10 is swapped with case 11.  The remainder are left invariant.

The second symmetry is where $j_1$ is swapped with $j_2$ and $j_3$ is
swapped with $j$.  Applying this to the defining relation for the
Racah coefficient, written as the recoupling relation as in equation
\ref{racah-discrete}, one finds the following transformations occur to
the Clebsch-Gordon coefficients (again a particular choice of basis
elements has been made):
\begin{multline*}
\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
j - m_{23} & m_{12} - j + m_{23} & m_{12}
\end{array} \right] 
\longmapsto\left[ \begin{array}{ccc} j_2 & j_1 & j_{12}\\ 
j_3 - m_{23} & m_{12} - j_3 + m_{23} & m_{12}
\end{array} \right] \\ =  
\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
m_{12} - j_3 + m_{23} & j_3 - m_{23} & m_{12}
\end{array} \right]
\end{multline*}
\begin{multline*}
\left[ \begin{array}{ccc} j_2 & j_3 & j_{23}\\ 
m_{12} - j + m_{23} & j-m_{12} & m_{23} 
\end{array} \right] 
\longmapsto\left[ \begin{array}{ccc} j_1 & j & j_{23}\\ 
m_{12} - j_3 +m_{23} & j_3 - m_{12} & m_{23} 
\end{array} \right]\\ = 
\left[ \begin{array}{ccc} j_1 & j_{23} & j\\ 
m_{12} - j_3 +m_{23} & -m_{23}  & - j_3 + m_{12}  
\end{array} \right]
\end{multline*}
$$
\left[ \begin{array}{ccc} j_1 & j_{23} & j\\ 
j - m_{23} & m_{23} & j \end{array} \right] 
\longmapsto\left[ \begin{array}{ccc} j_2 & j_{23} & j_{3}\\ 
j_3 - m_{23} & m_{23} & j_3 \end{array} \right] = 
\left[ \begin{array}{ccc} j_2 & j_3 & j_{23}\\ 
j_3 - m_{23} & -j_3 & -m_{23} \end{array} \right]
$$
$$
\left[ \begin{array}{ccc} j_{12} & j_3 & j\\ 
m_{12} & - m_{12} + j & j \end{array} \right] 
\longmapsto\left[ \begin{array}{ccc} j_{12} & j & j_3\\ 
m_{12} & - m_{12} + j_3 & j_3 \end{array} \right]\\  = 
\left[ \begin{array}{ccc} j_{12} & j_3 & j\\ 
m_{12} &  -j_3 & m_{12} - j_3 \end{array} \right]
$$

The final equalities will not be justified here since they, and
symmetries like them, are the subject of section \ref{inv}, although
it is possible to verify them directly for the cases where all
representations are in the discrete series from the defintions of the
Clebsch-Gordon coefficients in equations \ref{cg} and \ref{cg2}.  In
essence they are the \su{1,1} analogue of the well known permutation
symmetries for the \su{2} Clebsch-Gordon coefficient\cite{AngMom}.

The above symmetry has the property that it induces the following
exchanges among the different cases of coupling in table
\ref{posneg-racah}: case 1 is swapped with case 6, case 2 is swapped
with case 3, case 4 is swapped with case 8, case 5 is swapped with
case 7, case 9 is swapped with case 10 and case 11 is swapped with
case 12.

It is now possible to generate all the twelve different cases of
coupling in table \ref{posneg-racah} using the formulae in equations
\ref{RacahSU11}, \ref{su11-5} and \ref{su11-11}.  
Using the above two symmetries equation \ref{RacahSU11} now covers
cases 1, 4, 6 and 8, equation \ref{su11-5} covers cases 2, 3, 5 and 7
with the remaining four cases covered by \ref{su11-11}.
This concludes the calculation of the Racah coefficient for all cases
of coupling in the discrete series.




==> Racah/racahdis.new.tex <==

\section{The Racah Coefficients for the Discrete Series} \label{rac}

In this section explicit calculations will be made for the case where
all the representations are in the discrete series.  In contrast to
section \ref{CGC} the Clebsch-Gordon coefficients will be exhibited in
the $SO\left(2\right)$ discrete basis since the calculations are
easier in this form and the Racah coefficient is basis independent as
discussed in section \ref{Racah}.

We shall start with two lemmas that will be of use later

\begin{lem} \label{lem1}
\begin{multline}
\frac{\G{a+1}}{\G{b+1}\G{c+1}} =\\ \sum_n
\frac{\G{a-b+1}\G{a-c+1}}
{\G{a-b-n+1}\G{a-c-n-1}\G{b+c-a+n-1}\G{n+1}}
\end{multline}
\end{lem}

Lemma \ref{lem1} follows from the addition theorem for binomial
coefficients by expanding both sides of $(a+b)^n (a+b)^m =
(a+b)^{n+m}$ and equating powers of $a$ and $b$ as in \cite{RacahI}.

One also has the following for $n\in\Z^+$
\begin{multline*}
\frac{\G{a+n}}{\G{a}} = \left(a+n-1\right)\left(a+n-2\right)\dots
\left(a+1\right) a\\
= \left(-1\right)^n\left(1-a-n\right)\left(2-a-n\right)\dots
\left(-a-1\right)\left(-a\right)
= \left(-1\right)^n\frac{\G{1-a}}{\G{1-a-n}}
\end{multline*}
so that the following analytic continuation for $\Gamma$
functions holds
\begin{lem}\label{lem2}
$$
\frac{\G{a+n}}{\G{a}} = \left(-1\right)^n\frac{\G{1-a}}{\G{1-a-n}}
$$
for $n\in\Z^+$, $a\in\C$
\end{lem}

Finally there is the Gauss summation formula\cite{HypGeo}
\begin{lem}\label{lem3}
$$
\sum_{n}\frac{\G{a+n}\G{b+n}\G{c}}{\G{a}\G{b}\G{c+n}\G{n+1}}
= \frac{\G{c}\G{c-a-b}}{\G{c-a}\G{c-b}}
$$
\end{lem}

From section \ref{rep} the positive discrete series is characterised
by the following action of the generators of \su{1,1} on the Hilbert
spaces $\mathcal{H}_j$ with basis $\{\ket{j,m} |\;
j,m\in\frac{1}{2}\N,\;\; m\ge j\}$
\begin{align*}
K_3\ket{j,m} & = m\ket{j,m}\\
K_\pm\ket{j,m} & = \pm\sqrt{(m\pm j)(m\mp j\pm 1)}\ket{j,m\pm 1}
\end{align*}
while the negative discrete series simply has $m\mapsto -m$.

The Clebsch-Gordon coefficients for the discrete series may be defined
as follows
\begin{equation}\label{CGC-def-O2}
\ket{j\left(j_1 j_2\right),m} = \sum_{m_1,m_2} \left[
\begin{array}{ccc} j_1 & j_2 & j\\ m_1 & m_2 & m \end{array} \right]
\ket{j_1,m_1}\otimes\ket{j_2,m_2}
\end{equation}
with $m = m_1 + m_2$.  An explicit formula for the Clebsch-Gordon
coefficient may be derived via a recursion relation in the manner of
Holman and Biedenharn's approach to the problem (see for instance
\cite{HoBi66} and \cite{HoBi68}). Their formula for the Clebsch-Gordon 
coefficient of coupling in the discrete series consists of the two
solutions $\left[\begin{array}{ccc} j_1 & j_2 & j
\\ m_1 & m_2 & m\end{array}\right]_+$ and 
$\left[\begin{array}{ccc} j_1 & j_2 & j
\\ m_1 & m_2 & m\end{array}\right]_-$ where
\begin{multline}\label{cg}
\left[\begin{array}{ccc} j_1 & j_2 & j
\\ m_1 & m_2 & m\end{array}\right]_+ = 
\delta_{m_1+m_2,m}\\ \times
\sqrt{\frac{\G{m-j+1}\G{m+j}\G{m_1-j_1+1}\G{j_1-j_2+j}\G{j_1+j_2+j-1}}
{\G{m_2-j_2+1}\G{j_2+m_2}\G{m_1+j_1}\G{-j_1+j_2+j}\G{-j_1-j_2+j+1}}}\\
\times\HypT{j_2+m_2}{-m_1+j_1}{m_2-j_2+1}{m_2-j-j_1+1}{m_2+j+j_1}{1}
\end{multline}
and
\begin{equation}\label{cg2}
\left[\begin{array}{ccc} j_1 & j_2 & j
\\ m_1 & m_2 & m\end{array}\right]_- = 
\left[\begin{array}{ccc} j_2 & j_1 & j
\\ -m_2 & -m_1 & -m\end{array}\right]_+
\end{equation}
The particular solution used depends on the case of coupling.

Here a slightly different normalisation to Holman and Beidenharn's
original formula is being used so that the specific formula satisfies
the orthonormality relations in equations \ref{CGC-orth} and
\ref{CGC-orth2},  specifically the usual factor of $\sqrt{2j-1}$ has
been omitted.  Note also that Holman and Beidenharn's formula has the
$j$'s as negative half integers, whereas in equation \ref{cg}
the $j$'s are the more usual positive half integers.

The generalised hypergeometric function\cite{HypGeo} is defined
via
$$
\HypT{a}{b}{c}{d}{e}{z}
= \sum_n \frac{\G{a+n}\G{b+n}\G{c+n}\G{d}\G{e}z^n}
{\G{a}\G{b}\G{c}\G{d+n}\G{e+n}\G{n+1}}
$$
and converges if $-a-b-c+d+e > 0$.


The discrete basis version of the recoupling identity in equation
\ref{racah} may be expressed as
\begin{multline}\label{racah-discrete}
\sum_{m_{12}} 
\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
m_1 & m_2 & m_{12} \end{array} \right]
\left[ \begin{array}{ccc} j_{12} & j_3 & j\\ 
m_{12} & m_3 & m \end{array} \right]\\
= \sum_{j_{23}\;m_{23}} (2j_{23}+1) 
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ j_3 & j & j_{23} 
\end{array}\right\}
\left[ \begin{array}{ccc} j_2 & j_3 & j_{23}\\
m_2 & m_3 & m_{23} \end{array} \right]
\left[ \begin{array}{ccc} j_1 & j_{23} & j\\ 
m_1 & m_{23} & m \end{array} \right]
\end{multline}
where $\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\  m_1 & m_2 &
m_{12} \end{array} \right]$ are the Clebsch-Gordon coefficients for
the coupling of two unitary irreducible representations of $SU(1,1)$. 

The discrete basis version of the orthonormality relations in equation
\ref{CGC-orth} now becomes
\begin{equation}
\sum_{m_1}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ m_1 & m-m_1 & m \end{array} \right]
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ m_1 & m-m_1 & m \end{array} \right]
 = \frac{1}{2j-1} 
\end{equation}
and this relation may be used to bring equation \ref{racah-discrete}
into the following form
\begin{multline} \label{racdef}
\sum_\beta\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
j-j_{23} & \beta & j-j_{23} +\beta \end{array} \right]
\left[ \begin{array}{ccc} j_{12} & j_3 & j\\ 
j-j_{23} +\beta & j_{23}-\beta & j \end{array} \right]
\left[ \begin{array}{ccc} j_2 & j_3 & j_{23}\\ 
\beta & j_{23}-\beta & j_{23} \end{array} \right]\\
= \left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
j_3 & j & j_{23} \end{array}\right\}
\left[ \begin{array}{ccc} j_1 & j_{23} & j\\ 
j-j_{23} & j_{23} & j \end{array} \right]
\end{multline}
where the choice $m_{23} = j_{23}$ has been made.

Depending on the case of coupling one then uses either of
$
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_\pm
$.  From \cite{HoBi68} one must
take
$$
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right] = 
\begin{cases}\renewcommand{\arraystretch}{0.7}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_+ & 
\text{ for }j_1,j_2,j_{12}\in\mathcal{D}^+\\
\renewcommand{\arraystretch}{0.7}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_- & 
\text{\parbox{5cm}{ for $j_1,j\in\mathcal{D}^+$, 
$j_2\in\mathcal{D}^-$\\[-3.5mm] $\,m \ge j_1-j_2$, $m>0$}}\\
\renewcommand{\arraystretch}{0.7}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_+ &
\text{\parbox{5cm}{ for $j_1\in\mathcal{D}^+$,
$j_2,j\in\mathcal{D}^-$\\[-3.5mm] $m \le j_1-j_2$, $m<0$}}\\
\renewcommand{\arraystretch}{0.7}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_- & 
\text{ for }j_1,j_2,j_{12}\in\mathcal{D}^- 
\end{cases}
$$

Now consider the representations $j_1$, $j_2$ and $j_3$.  Formally
there are $2^3 = 8$ different combinations of positive and negative
discrete representations, however these come in dual pairs so there
are only four unique possibilities.  It is now a simply matter to
enumerate the possibilities for the remaining discrete series
representations in the Racah coefficent in table \ref{posneg-racah}.

\begin{table}[hbt!]
\begin{center}
\begin{tabular}{ccccccc}
Case & $j_1$ & $j_2$ & $j_3$ & $j_{12}$ & $j_{23}$ & $j$\\
(1) & + & + & + & + & + & +\\
(2) &$-$& + & + & + & + & +\\
(3) &$-$& + & + &$-$& + & +\\
(4) &$-$& + & + &$-$& + &$-$\\
(5) & + & + &$-$& + & + & +\\
(6) & + & + &$-$& + &$-$&$-$\\
(7) & + & + &$-$& + &$-$& +\\
(8) &$-$& + &$-$& + & + & +\\
(9) &$-$& + &$-$& + & + &$-$\\
(10)&$-$& + &$-$&$-$& + &$-$\\
(11)&$-$& + &$-$& + &$-$&$-$\\
(12)&$-$& + &$-$&$-$&$-$&$-$\\
\end{tabular}
\end{center}
\caption{The possible unique distributions of positive and negative discrete 
representations in the Racah coefficient\label{posneg-racah}}
\end{table}

Consider the Clebsch-Gordon coefficient on the right hand side of
equation \ref{racdef}.  One has
$$
\left[\begin{array}{ccc}
j_1 & j_{23} & j\\
m_1 & j_{23} & j
\end{array}\right] = 
\begin{cases}
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & m_1 & j_{23}+m_1
\end{array}\right]_+ & \text{for cases 1 and 5}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
-j_{23} & -m_1 & -j_{23}-m_1
\end{array}\right]_- & \text{for cases 11 and 12}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & -m_1 & j_{23}-m_1
\end{array}\right]_- & \text{for cases 2, 3 and 8}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & -m_1 & j_{23}-m_1
\end{array}\right]_+ & \text{for cases 4, 9 and 10}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_1 & j_{23} & j\\
m_1 & -j_{23} & m_1-j_{23}
\end{array}\right]_+ & \text{for case 6}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_1 & j_{23} & j\\
m_1 & -j_{23} & m_1-j_{23}
\end{array}\right]_- & \text{for case 7}\\
\end{cases}
$$

Now note that by equation \ref{cg2} there are only three unique
evaluations to be made since 
$$
\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & m_1 & j_{23}+m_1
\end{array}\right]_+ = \left[\begin{array}{ccc}
j_{23} & j_1 & j\\
-j_{23} & -m_1 & -j_{23}-m_1
\end{array}\right]_-
$$
and cases 1, 5, 11 and 12 are equivalent here, also
$$\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & -m_1 & j_{23}-m_1
\end{array}\right]_- = \left[\begin{array}{ccc}
j_1 & j_{23} & j\\
m_1 & -j_{23} & m_1-j_{23}
\end{array}\right]_+
$$
so that cases 2, 3, 6 and 8 have the same Clebsch-Gordon coefficient,
and
$$
\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & -m_1 & j_{23}-m_1
\end{array}\right]_+ = \left[\begin{array}{ccc}
j_1 & j_{23} & j\\
m_1 & -j_{23} & m_1-j_{23}
\end{array}\right]_-
$$
allowing cases 4, 7, 9 and 10 to be treated together.

For these last for cases the value of $m_1$ will be fixed as $m_1 =
j_1$, while for the first four cases, 1, 5, 11 and 12, take $m_1 =
j-j_{23}$.  The remaining four cases have $m_1 = j_{23}-j$.

In the following any constant phase may, and will, be discarded since
the phase of the Racah coefficient is arbitrary.  Hence all the
equalities are modulo a phase.  In addition the $\Gamma$ functions may
need to be understood in terms of their analytic continuations via
lemma \ref{lem2}, depending on the specifics of the cases of coupling.

By direct evaluation one may show, for cases 1, 2, 3, 5, 6, 8, 11 and
12,
\begin{multline}
\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & j-j_{23} & j
\end{array}\right]_+ = \left[\begin{array}{ccc}
j_1 & j_{23} & j\\
-j+j_{23} & -j_{23} & -j
\end{array}\right]_+\\
 = \sqrt{\frac{\G{j_{23}+j-j_1}\G{j+j_1+j_{23}-1}}{\G{2j}\G{2j_{23}}}}
\end{multline}

The result for $\left[\begin{array}{ccc}
j_1 & j_{23} & j\\
j-j_{23} & j_{23} & j
\end{array}\right]_+$ follows immediately from equation \ref{cg} and
the fact that 
$$
\sum_{n\in\Z}
\frac{A\left(n\right)}{\G{1-r+n}\G{1+r-n}} = A\left(r\right)
$$
for $r\in\Z$

The other evaluation requires the Gauss summatation formula (lemma
\ref{lem3}) to evaluate the sum in the hypergeometric series and
repeated applications of lemma \ref{lem2} to bring it into the same
form.

For the remaining cases, 4,7,9 and 10, one has
\begin{multline}
\left[\begin{array}{ccc}
j_1 & j_{23} & j\\
j_1 & -j_{23} & j_1-j_{23}
\end{array}\right]_- = \left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & -j_1 & j_{23}-j_1
\end{array}\right]_- \\
 = \sqrt{\frac{\G{j_{23}-j+j_1}\G{j+j_1+j_{23}-1}}{\G{2j}\G{2j_{23}}}}
\end{multline}
again by a direct evaluation and repeated use of lemma \ref{lem2}.


Similarly consider the Clebsch-Gordon coefficient that determines the
coupling of $j_2$ and $j_3$. Once the cases that are dual to each
other have been combined one has again three cases
\begin{equation}
\left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
\beta & j_{23}-\beta & j_{23}
\end{array}\right] = 
\begin{cases}
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
\beta & j_{23}-\beta & j_{23}
\end{array}\right]_+ & \text{for cases 1, 2, 3 and 4}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
\beta & -j_{23}-\beta & -j_{23}
\end{array}\right]_+ & \text{for cases 6, 7, 11 and 12}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
\beta & j_{23}-\beta & j_{23}
\end{array}\right]_- & \text{for cases 5, 8, 9 and 10}
\end{cases}
\end{equation}

Again, a direct evaluation in the same manner as the previous case
shows that two of these are equal. Thus for cases 1, 2, 3, 4, 5, 8, 9,
and 10 it may be may be evaluated as
\begin{multline}
\left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
\beta & j_{23}-\beta & j_{23}
\end{array}\right]_+ = \left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
\beta & j_{23}-\beta & j_{23}
\end{array}\right]_-
\\ = 
\frac{\left(-1\right)^b\Delta\left(j_2 j_3 j_{12}\right)}
{\sqrt{\G{2j_{23}}\G{\beta+j_2}\G{j_{23}-j_3-\beta+1}}}\\
\times\frac{1}{\sqrt{\G{\beta-j_2+1}\G{j_3+j_{23}-\beta}}}
\end{multline}
where
\begin{multline*}
\Delta\left(j_1 j_2 j_{12}\right) = \sqrt{
\G{j_1+j_2+j-1}\G{-j_1+j_2+j}}\\
\times\sqrt{\G{j_1-j_2+j}\G{-j_1-j_2+j+1}}
\end{multline*}

The third, covering cases 6, 7, 11 and 12, may be evaluated as
\begin{multline}
\left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
\beta & -j_{23}-\beta & -j_{23}
\end{array}\right]_+ = \left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
-\beta & j_{23}+\beta & j_{23}
\end{array}\right]_+\\ = 
\frac{\left(-1\right)^b\Delta\left(j_2 j_3 j_{12}\right)}
{\sqrt{\G{2j_{23}}\G{\beta+j_2}\G{j_{23}-j_3+\beta+1}}}\\
\times\frac{1}{\sqrt{\G{-\beta-j_2+1}\G{j_3+j_{23}+\beta}}}
\end{multline}

Next, consider the Clebsch-Gordon coefficient 
$\left[\begin{array}{ccc}
j_{12} & j_3 & j\\
j-j_{23}+\beta & j_{23}-\beta & j
\end{array}\right]$. After combining cases related by equation
\ref{cg2} and making sure to preserve the assignments made to $m_1$
\begin{multline}
\left[\begin{array}{ccc}
j_{12} & j_3 & j\\
j-j_{23}+\beta & j_{23}-\beta & j
\end{array}\right] =\\ 
\begin{cases}
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_3 & j_{12} & j\\
j_{23}-\beta & j-j_{23}+\beta & j
\end{array}\right]_+ & \text{for cases 1 and 2}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_3 & j_{12} & j\\
j_{23} - \beta& \beta-j_{23}+j & j
\end{array}\right]_- & \text{for cases 3, 5 and 8}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_3 & j_{12} & j\\
j_{23}-\beta & -j_1 +\beta & j_{23}-j_1
\end{array}\right]_- & \text{for cases 4, 9 and 10}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_{12} & j_3 & j\\
-j+j_{23}+\beta & -j_{23}-\beta & -j
\end{array}\right]_+ & \text{for cases 6, 11 and 12}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_{12} & j_3 & j\\
j_1+\beta & -j_{23} -\beta & -j_{23}+j_1
\end{array}\right]_- & \text{for case 7}
\end{cases}
\end{multline}

Direct evaluation as in the previous two cases yields the following
explicit formulae for cases 1, 2, 3, 5 and 8
\begin{multline}
\left[\begin{array}{ccc}
j_3 & j_{12} & j\\
j_{23}-\beta & j-j_{23}+\beta & j
\end{array}\right]_+ = \left[\begin{array}{ccc}
j_3 & j_{12} & j\\
j_{23}-\beta & j-j_{23}+\beta & j
\end{array}\right]_-\\
= \frac{\left(-1\right)^\beta\Delta\left(j_3j_{12}j\right)}
{\sqrt{\G{2j}\G{j-j_{23}-j_{12}+\beta+1}\G{j_{12}+j-j_{23}+\beta}}}\\
\times\frac{1}{\sqrt{\G{j_{23}-\beta-j_3+1}\G{j_3+j_{23}-\beta}}}
\end{multline}

and, for cases 6, 11 and 12,

\begin{multline}
\left[\begin{array}{ccc}
j_{12} & j_3 & j\\
-j+j_{23}+\beta & -j_{23}-\beta & -j
\end{array}\right]_+ \\
= \frac{\left(-1\right)^\beta\Delta\left(j_3j_{12}j\right)}
{\sqrt{\G{2j}\G{j-j_{23}-j_{12}-\beta+1}\G{j_{12}+j-j_{23}-\beta}}}\\
\times\frac{1}{\sqrt{\G{j_{23}+\beta-j_3+1}\G{j_3+j_{23}+\beta}}}
\end{multline}

The remaining four cases remain as sums and one has, for cases 4, 9
and 10,
\begin{multline}
\left[\begin{array}{ccc}
j_3 & j_{12} & j\\
j_{23}-\beta & \beta-j_1 & j_{23}-j_1
\end{array}\right]_- = \frac{\Delta\left(j_3 j_{12}j\right)}
{\G{j_3+j-j_{12}}\G{j-j_{12}-j_3+1}}\\ \times
\sqrt{\frac{\G{j_1-j_{23}-j+1}\G{j_1-j_{23}+j}\G{j_1-j_{12}+1-\beta}}
{\G{1-j_3-j_{23}+\beta}\G{j_3-j_{23}+\beta}\G{j_1+j_2-\beta}}}\\ \times
\sum_n\frac{\left(-1\right)^n\G{j_{12}-j_1-\beta+n}\G{-j_1-j_{12}-\beta+1+n}}
{\G{-j_1-\beta-j+j_3+1+n}\G{-j_1-\beta+j+j_3+n}}\\ \times
\frac{1}{\G{1+j_{23}-j_3+\beta-n}\G{n+1}}
\end{multline}
and for case 7,
\begin{multline}
\left[\begin{array}{ccc}
j_{12} & j_3 & j\\
j_1 + \beta & -j_{23}-\beta & j_1-j_{23}
\end{array}\right]_- = \frac{\Delta\left(j_3 j_{12} j\right)}
{\G{j+j_{12}-j_3}\G{j-j_{12}-j_3+1}}\\ \times
\sqrt{\frac{\G{j_{23}-j_1-j+1}\G{j_{23}-j_1+j}\G{j_{23}+\beta-j_3+1}}
{\G{-j_1-j_{12}-\beta+1}\G{j_{12}-j_1-\beta}\G{j_{23}+\beta+j_3}}}\\
\times\sum_n\frac{\left(-1\right)^n\G{j_{12}-j_1-\beta+n}
\G{-j_1-\beta-j_{12}+1+n}}{\G{-j_1-\beta-j+j_3+1+n}\G{-j_1-\beta+j+j_3+n}}
\\ \times
\frac{1}{\G{1+j_{23}+\beta-j_3-n}\G{n+1}}
\end{multline}

The final Clebsch-Gordon coefficient to consider is $
\left[\begin{array}{ccc}
j_1 & j_2 & j_{12}\\ j-j_{23} & \beta & j-j_{23}+\beta
\end{array}\right]$.   After cases of coupling that are equivalent by
equation \ref{cg2} are combined one has
\begin{multline}
\left[\begin{array}{ccc}
j_1 & j_2 & j_{12}\\ j-j_{23} & \beta & j-j_{23}+\beta
\end{array}\right]\\ = 
\begin{cases}
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & j-j_{23} & j-j_{23}+\beta
\end{array}\right]_+ & \text{for cases 1, 5 and 12}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & j_{23}-j & j_{23}-j+\beta
\end{array}\right]_+ & \text{for cases 3 and 6}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & j-j_{23} & j-j_{23}+\beta
\end{array}\right]_- & \text{for cases 2, 8 and 11}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & j_1 & j_1+\beta
\end{array}\right]_+ & \text{for case 7}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & -j_{1} & -j_{1}+\beta
\end{array}\right]_- & \text{for case 9}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & -j_{1} & -j_{1}+\beta
\end{array}\right]_+ & \text{for cases 4 and 10}\\
\end{cases}
\end{multline}

As before a direct evaluation of these Clebsch-Gordon coefficients
yields, for cases 4, 9 and 10,
\begin{multline}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & -j_{1} & -j_{1}+\beta
\end{array}\right]_+ = \left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & -j_{1} & -j_{1}+\beta
\end{array}\right]_-\\
= \frac{\Delta\left(j_1 j_2 j_{12}\right)}
{\sqrt{\G{2j_1}\G{j_{12}-j_1-j_2+1}\G{-j_1+j_2+j_{12}}}}\\
\times\sqrt{\frac{\G{\beta-j_1-j_2+1}\G{\beta-j_1+j_{12}}}
{\G{\beta-j_2+1}\G{\beta+j_2}}}
\end{multline}

For case 7,
\begin{multline}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & j_1 & j_1+\beta
\end{array}\right]_+ =  \frac{\Delta\left(j_1 j_2 j_{12}\right)}
{\sqrt{\G{2j_1}\G{j_{12}-j_1-j_2+1}\G{-j_1+j_2+j_{12}}}}\\
\times\sqrt{\frac{\G{\beta-j_2+1}\G{\beta+j_{2}}}
{\G{\beta+j_1-j_2+1}\G{\beta+j_1+j_{12}}}}
\end{multline}

The remaining cases are only expressible as sums. One has, for cases
2, 8 and 11,
\begin{multline}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & j-j_{23} & \beta+j-j_{23}
\end{array}\right]_+ = \frac{\Delta\left(j_1 j_2 j_{12}\right)}
{\sqrt{\G{j_1+j_{12}-j_2}\G{j_{12}-j_1-j_2+1}}}\\ \times
\sqrt{\frac{\G{\beta+j-j_{23}-j_{12}+1}
\G{-j_{23}+\beta+j+j_{12}}\G{\beta-j_2+1}}
{\G{\beta+j_2}\G{j_{23}-j_1-j+1}\G{j_1-j_{23}+j}}}\\ \times
\sum_n\frac{\left(-1\right)^n\G{j_1-j_{23}+j+n}\G{j-j_{23}-j_1+1+n}}
{\G{j-j_{23}-j_{12}+j_2+1+n}\G{j-j_{23}+j_{12}+j_2+n}
\G{1+\beta-j_2-n}\G{n+1}}
\end{multline}

For cases 1, 5 and 12,
\begin{multline}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & -j+j_{23} & \beta-j+j_{23}
\end{array}\right]_+ = \frac{\Delta\left(j_1 j_2 j_{12}\right)}
{\sqrt{\G{j_1+j_{12}-j_2}\G{j_{12}-j_1-j_2+1}}}\\ \times
\sqrt{\frac{\G{\beta+j_{23}+j-j_{12}+1}
\G{j_{23}+\beta-j+j_{12}}\G{\beta-j_2+1}}
{\G{\beta+j_2}\G{j_{23}+j_1-j}\G{-j_1+j_{23}-j+1}}}\\ \times
\sum_n\frac{\left(-1\right)^n\G{j_1+j_{23}-j+n}\G{j_{23}-j-j_1+1+n}}
{\G{j_{23}-j-j_{12}+j_2+1+n}\G{j_{23}-j+j_{12}+j_2+n}
\G{1+\beta-j_2-n}\G{n+1}}
\end{multline}

and finally for cases 3 and 6
\begin{multline}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & j-j_{23} & \beta+j-j_{23}
\end{array}\right]_- = \frac{\Delta\left(j_1 j_2 j_{12}\right)}
{\sqrt{\G{j_1+j_{12}-j_2}\G{j_{12}-j_1-j_2+1}}}\\ \times
\sqrt{\frac{\G{j_{23}-\beta-j-j_{12}+1}
\G{j_{23}-j-\beta+j_{12}}\G{j_{23}-j_1-j+1}}
{\G{1-\beta-j_2}\G{j_{23}+j_1-j}\G{-\beta+j_2}}}\\ \times
\sum_n\frac{\left(-1\right)^n\G{-\beta+j_2+n}\G{-\beta-j_2+1+r}}
{\G{j_1-j_{12}-\beta+1+n}\G{j_1+j_{12}-\beta+n}
\G{1-j_1+j_{23}-j-n}\G{n+1}}
\end{multline}

It now remains to calculate the Racah cofficient for the twelve cases
given in table \ref{posneg-racah}.  

First note that cases 1 and 5 may be grouped together since the
Clebsch-Gordon coefficients have been shown to have exactly the same
form for these two cases.  Thus the resulting Racah coefficient
consists of one equation that may be analytically continued, using
lemma \ref{lem3}, to the respective domains of definition.  In a
similar way cases 4, 9 and 10 may be combined, as may cases 2 and 8.

Explicitly the calculation for cases 1 and 5 proceeds from a
substitution of equation
\ref{cg} into \ref{racdef}, which gives the following
\begin{multline} \label{rac2}
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ j_3 & j & j_{23} \end{array} 
\right\} = \frac{\Delta\left(j_2 j_3 j_{23}\right)
\Delta\left(j_{12}j_3 j\right)\Delta\left(j_1 j_{23} j\right)}
{\sqrt{\G{j_1+j-j_{23}}\G{-j_1+j+j_{23}}\G{j_1+j+j_{23}-1}}}\\
\times\frac{\Delta\left(j_1 j_2 j_{12}\right)\,\mathcal{I}}
{\sqrt{\G{-j_1+j_2+j_{12}}\G{-j_1-j_2+j_{12}-1}}}
\end{multline}
where
\begin{multline*}
\mathcal{I} =
\sum_{\beta\,r}
\frac{\left(-1\right)^{r+j-j_{23}+2\beta-j_{12}-j_2}
\G{j_2+\beta+r}\G{\beta-j_2+1+r}}
{\G{j_2+\beta}\G{\beta -j_{12}+j_1+1+r}}\\
\times\frac{1}
{\G{\beta+j_{12}+j_1+r}\G{1+j-j_{23}-j_1-r}\G{k_{23}-\beta -k_3+1}}\\
\times\frac{1}{\G{k_3+k_{23}-\beta}\G{\beta-k_2+1}\G{r+1}}
\end{multline*}

$\mathcal{I}$ may be reduced to a single summation as
follows. Introduce a new summation using lemma \ref{lem1} with $a =
j_2+\beta+r-1$, $b=\beta-j_{12}+j_1+r$ and $c = \beta+k_{12}
+k_1+r-1$, one has
\begin{multline}\label{SumI}
\mathcal{I} = 
\sum_{\beta\,r\,s}
\frac{\left(-1\right)^{r+j-j_{23}+2\beta-j_{12}-j_2}
\G{\beta-j_2+1+r}}
{\G{j_2+\beta}\G{k_3+k_{23}-\beta}\G{1+j-j_{23}-j_1-r}}\\
\times\frac{1}
{\G{\beta+2j_1+r+1-j_2+s}
\G{j_{23}-\beta -j_3+1}\G{\beta-j_2+1}\G{r+1}}\\
\times\frac{\G{j_2+j_{12}-j_1}\G{j_2-j_{12}-j_1+1}}
{\G{j_2+j_{12}-j_1-s}\G{j_2-j_{12}-j_1+1-s}\G{s+1}}
\end{multline}

Now the sum over $r$
$$
\sum_{r}\frac{\left(-1\right)^{r}\G{\beta-j_2+1+r}}
{\G{r+1}\G{1+j-j_{23}-j_1-r}\G{\beta+2j_1+r+1-j_2+s}}
$$
may be written, using the analytic continuation of lemma \ref{lem2}, as
\begin{multline*}
\sum_{r}\frac{\G{\beta-j_2+1+r}\G{-j+j_{23}+j_1+r}
\G{1+j-j_{23}-j_1}}
{\G{r+1}\G{\beta+2j_1+r+1-j_2+s}\G{-j+j_{23}+j_1}}\\
= \frac{\G{\beta-j_2+1}\G{j_1+j-j_{23}+s}}
{\G{j_1-j_2+j-j_{23}+s+\beta+1}\G{2k_1+s}}
\end{multline*}
and evaluated using lemma \ref{lem3}.  Substituting back into
equation \ref{SumI} gives
\begin{multline}\label{SumII}
\mathcal{I} = \sum_{\beta\,s}
\frac{\left(-1\right)^{j-j_{23}+2\beta-j_{12}-j_2}\G{j_1+j-j_{23}+s}}
{\G{j_2+\beta}\G{j_3+j_{23}-\beta}\G{j_{23}-\beta -j_3+1}
\G{j_2-j_{12}-j_1+1-s}}\\
\times\frac{\G{j_2+j_{12}-j_1}\G{j_2-j_{12}-j_1+1}}
{\G{j_1-j_2+j-j_{23}+s+\beta+1}
\G{j_2+j_{12}-j_1-s}\G{2j_1+s}\G{s+1}}
\end{multline}

Now note that the basis label $\beta$ is integer or half integer
according to the whether the representation label $j_2$ is integer or
half integer, respectively, and the sum is over integers or half
integers only.  Hence it makes no difference if the phase given by the
exponent $j-j_{23}+2\beta-j_{12}-j_2$ is now given by the exponent
$j-j_{23}+j_2-j_{12}$.

The sum over $\beta$ is now
\begin{multline*}
\sum_\beta
\frac{1}{\G{j_2+\beta}\G{j_3+j_{23}-\beta}}\\ \times
\frac{1}{\G{j_{23}-\beta -j_3+1}\G{j_1-j_2+j-j_{23}+s+\beta+1}}
\end{multline*}
and setting $z+1 = j_2+\beta$ this may be evaluated using lemma
\ref{lem1}
\begin{multline*}
\sum_z
\frac{1}{\G{z+1}\G{j_3+j_{23}+j_2-z-1}\G{j_{23} -j_3+j_2-z}}\\
\frac{1}{\G{j_1-2j_2+j-j_{23}+s+2+z}}
=\frac{\G{j_1+j+j_{23}+s+2}}
{\G{j_3+j_2+j_{23}+1}\G{j_{23}-j_3+j_2}}\\
\times\frac{1}{\G{j_1+j-j_2+j_3+s+2}\G{j_1+j-j_2-j_3+s+1}}
\end{multline*}
subsitituting this back into equation \ref{SumII} the final result is
gained (the phase is arbitary and so discarded)
\begin{multline}\label{RacahSU11}
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ j_3 & j & j_{23} \end{array} 
\right\} = \frac{\Delta\left(j_2 j_3 j_{23}\right)
\Delta\left(j_{12}j_3 j\right)\Delta\left(j_1 j_{23} j\right)}
{\G{j_1+j-j_{23}}\G{-j_1+j+j_{23}}\G{j_1+j+j_{23}-1}}\\
\times\frac{\Delta\left(j_1 j_2 j_{12}\right)
\G{j_2+j_{12}-j_1}\G{j_2-j_{12}-j_1+1}}
{\G{-j_1+j_2+j_{12}}\G{-j_1-j_2+j_{12}-1}
\G{j_3+j_2+j_{23}+1}\G{j_{23}-j_3+j_2}}\\ \times
\sum_{s}\frac{\G{j_1+j-j_{23}+s}\G{j_1+j+j_{23}+s-1}}
{\G{j_2-j_{12}-j_1+1-s}\G{j_1+j-j_2+j_3+s}\G{j_2+j_{12}-j_1-s}}\\
\times\frac{1}{\G{j_1+j-j_2-j_3+s+1}\G{2j_1+s}\G{s+1}}
\end{multline}
Writing this in terms of a generalised hypergeometric function
\begin{multline}\label{Racah-Su11-hyper}
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}
\\ j_3 & j & j_{23} \end{array} \right\} 
= \frac{\Delta\left(j_1 j_2 j_{12}\right)
\Delta\left(j_{12}j_3j\right)}{\G{j_2-j_1+j_{12}}\G{j_{12}-j_1-j_2+1}}\\
\times\frac{\Delta\left(j_2 j_3 j_{23}\right)
\Delta\left(j_1 j_{23} j\right)}
{\G{j_{23}+j_2-j_3}\G{j_2+j_3+j_{23}-1}
\G{j-j_{23}-j_1+1}\G{j+j_{23}-j_1}}\\ \times
\frac{1}{\G{2j_1}\G{j+j_1-j_2-j_3+1}\G{-j_2+j_1+j_3+j}}\\ \times
\HypF{j_1+j-j_{23}}{j_{23}+j_1+j-1}{1-j_2-j_{12}+j_1}{-j_2+j_{12}+j_1}
{2j_1}{j_1+j-j_2-j_3+1}{j_1-j_2+j_3+j}{1}
\end{multline}

\bigskip

The strategy for evaluating the remaining cases is similar and the
details will be omitted in favour of the end realisation of the Racah
coefficient in terms of a generalised ${ }_4F_3$ hypergeometric
function which covers the relevant cases using the analytic
continuations of lemma \ref{lem2} as necessary.

As discussed previously, cases 4, 9 and 10 may also be treated
together. These then give the result
\begin{multline}
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}
\\ j_3 & j & j_{23} \end{array} \right\} 
= \frac{\Delta\left(j_2 j_{12}j_1\right)\Delta\left(j_3jj_{12}\right)}
{\G{j_3+j_{23}-j_2}\G{-j_3+j_{23}-j_2+1}}\\
\times\frac{\Delta\left(j_2 j_3 j_{23}\right)
\Delta\left(j_{23} j j_1\right)}
{\G{j_1+j_{12}-j_2}\G{j_1+j_{23}+j-1}
\G{j_{12}+j-j_{23}+j_2}\G{j_{23}+j_1-j}}\\ \times
\frac{1}{\G{2j_2}\G{1+j_1-j_{12}-j_2}\G{-j_{23}+j_2-j+j_{12}+1}}\\ \times
\HypF{-j_{23}+j_2+j_3}{-j_{23}+j_2-j_3+1}{j_2+j_{12}+j_1-1}{-j_1+j_{12}+j_2}
{2j_2}{-j_{23}+j_2-j+j_{12}+1}{j_{12}+j-j_{23}+j_2}{1}
\end{multline}
and case 7 may be derived as
\begin{multline}
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}
\\ j_3 & j & j_{23} \end{array} \right\} 
= \frac{\Delta\left(j_2 j_1 j_{12}\right)\Delta\left(j j_3 j_{12}\right)}
{\G{j_3+j_{23}-j_2}\G{j-j_3+j_{12}}}\\
\times\frac{\Delta\left(j_2 j_{23} j_3\right)
\Delta\left( j j_{23} j_1\right)}
{\G{j_{12}-j_1-j_2+1}\G{j_1+j+j_{23}-1}
\G{j_3-j_2-j_{23}+1}\G{j_{23}-j+j_1}}\\ \times
\frac{\G{j_{23}-j-j_1+1}\G{j_{23}+j-j_1}}
{\G{j_2+j_3-j-j_1+1}\G{j+j_2+j_3-j_1}}\\ 
\times\frac{1}
{\G{2j_2}\G{j_{12}-j_3-j+1}\G{j_1-j_2+j_{12}}}\\
\HypF{j_{12}-j_1+j_2}{j_2-j_1-j_{12}+1}{j_2+j_3+j_{23}-1}{j_2+j_3-j_{23}}
{j_2+j_3-j_1-j+1}{j_2+j_3-j_1+j}{2j_2}{1}
\end{multline}

Consider now the following symmetry, where $j_{12}$ is swapped with
$j_{23}$ and $j_1$ is swapped with $j_2$, applied to equation
\ref{racdef}.  One now has
\begin{multline}
\sum_\beta\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
j-m_{23} & \beta & j-m_{23} +\beta \end{array} \right]
\left[ \begin{array}{ccc} j_1 & j_{23} & j\\ 
j-m_{23} & m_{23} & j \end{array} \right]
\left[ \begin{array}{ccc} j_2 & j_3 & j_{23}\\ 
\beta & m_{23}-\beta & m_{23} \end{array} \right]\\
= \left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
j_3 & j & j_{23} \end{array}\right\}
\left[ \begin{array}{ccc} j_{12} & j_3 & j\\ 
j-m_{23} +\beta & m_{23}-\beta & j \end{array} \right]
\end{multline}
This equation is the defining relation for a Racah coefficient with a
potentially different distribution of positive and negative discrete
series.  In particular it is easy to see from table \ref{posneg-racah}
that it transforms case 5 into case 2, case 4 into case 6, case 10
into case 11 and case 7 into case 3 (and vice versa).  Hence formulae
for cases 2, 3, 6, 8 and 11 may be derived by simply transforming the
appropriate formula for the related case by this symmetry.

Finally to deal with case 12 one needs another symmetry.  Here $j_1$
is swapped with $j_2$ and $j_3$ is swapped with $j$.  Applying this to
the defining relation for the Racah coefficient for case 12 one finds
the following transformations occur to the Clebsch-Gordon
coefficients:
$$
\begin{array}{ccccc}
\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
m_1 & m_2 & m_{12} \end{array} \right] &
\longmapsto & \left[ \begin{array}{ccc} j_2 & j_1 & j_{12}\\ 
m_2 & m_1 & m_{12} \end{array} \right] & = & 
\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
m_1 & m_2 & m_{12} \end{array} \right]\\
\left[ \begin{array}{ccc} j_2 & j_3 & j_{23}\\ 
m_2 & m_3 & m_{23} \end{array} \right] &
\longmapsto & \left[ \begin{array}{ccc} j_1 & j & j_{23}\\ 
m_1 & m & m_{23} \end{array} \right] & = &
\left[ \begin{array}{ccc} j_1 & j_{23} & j\\ 
m_1 & -m_{23} & -m \end{array} \right]\\
\left[ \begin{array}{ccc} j_1 & j_{23} & j\\ 
m_1 & m_{23} & m \end{array} \right] &
\longmapsto & \left[ \begin{array}{ccc} j_2 & j_{23} & j_{3}\\ 
m_2 & m_{23} & m_3 \end{array} \right] & = & 
\left[ \begin{array}{ccc} j_2 & j_3 & j_{23}\\ 
m_2 & -m_3 & -m_{23} \end{array} \right]\\
\left[ \begin{array}{ccc} j_{12} & j_3 & j\\ 
m_{12} & m_3 & m \end{array} \right] &
\longmapsto & \left[ \begin{array}{ccc} j_{12} & j & j_3\\ 
m_{12} & m & m_3 \end{array} \right] & = &
\left[ \begin{array}{ccc} j_{12} & j_3 & j\\ 
m_{12} & -m_3 & -m \end{array} \right]
\end{array}
$$
The final equalities will not be justified here since they, and
symmetries like them, are the subject of section \ref{inv}.  In
essence they are the \su{1,1} analogue of the well known permutation
symmetries for the \su{2} Clebsch-Gordon coefficient\cite{AngMom}.

Applying this symmetry to case 12 yields the dual case (where all
positive discrete series go to negative discrete series and vice
versa) to case 11, for which a formula has already been derived.  This
then completes the calculation of the Racah coefficient for all cases
of coupling in the discrete series.


==> Racah/racahdis.tex <==

\section{The Racah Coefficients for the Discrete Series} \label{rac}

In this section explicit calculations will be made for the case where
all the representations are in the discrete series.  In contrast to
section \ref{CGC} the Clebsch-Gordon coefficients will be exhibited in
the $SO\left(2\right)$ discrete basis since the calculations are
easier in this form and the Racah coefficient is basis independent as
discussed in section \ref{Racah}.

We shall start with two lemmas that will be of use later

\begin{lem} \label{lem1}
\begin{multline}
\frac{\G{a+1}}{\G{b+1}\G{c+1}} =\\ \sum_n
\frac{\G{a-b+1}\G{a-c+1}}
{\G{a-b-n+1}\G{a-c-n-1}\G{b+c-a+n-1}\G{n+1}}
\end{multline}
\end{lem}

Lemma \ref{lem1} follows from the addition theorem for binomial
coefficients by expanding both sides of $(a+b)^n (a+b)^m =
(a+b)^{n+m}$ and equating powers of $a$ and $b$ as in \cite{RacahI}.

One also has the following for $n\in\Z^+$
\begin{multline*}
\frac{\G{a+n}}{\G{a}} = \left(a+n-1\right)\left(a+n-2\right)\dots
\left(a+1\right) a\\
= \left(-1\right)^n\left(1-a-n\right)\left(2-a-n\right)\dots
\left(-a-1\right)\left(-a\right)
= \left(-1\right)^n\frac{\G{1-a}}{\G{1-a-n}}
\end{multline*}
so that the following analytic continuation for $\Gamma$
functions holds
\begin{lem}\label{lem2}
$$
\frac{\G{a+n}}{\G{a}} = \left(-1\right)^n\frac{\G{1-a}}{\G{1-a-n}}
$$
for $n\in\Z^+$, $a\in\C$, $a\not\in\Z$
\end{lem}
as a consequence to lemma \ref{lem2} the following holds
\begin{equation}\label{an-cont}
\frac{\G{a}\G{1-a}}{\G{b}\G{1-b}} = \left(-1\right)^{a-b}
\end{equation}
for $a,b\in\Z^+$.  To see this note that from \ref{lem2} one has for
$k\in\C$, $k\not\in\Z$.
$$
\frac{\G{a+k}\G{1-a-k}}{\G{b+k}\G{1-b-k}}
= \frac{\G{k}\G{1-k}}{\G{k}\G{1-k}}\left(-1\right)^{a-b}
= \left(-1\right)^{a-b}
$$
now let $k\to 0$ and since the right hand side is independent of $k$
one may remove the requirement $k\not\in\Z$ and the equation becomes
equation \ref{an-cont}.

Finally there is the Gauss summation formula\cite{HypGeo}
\begin{lem}\label{lem3}
$$
\sum_{n}\frac{\G{a+n}\G{b+n}\G{c}}{\G{a}\G{b}\G{c+n}\G{n+1}}
= \frac{\G{c}\G{c-a-b}}{\G{c-a}\G{c-b}}
$$
\end{lem}

From section \ref{rep} the positive discrete series is characterised
by the following action of the generators of \su{1,1} on the Hilbert
spaces $\mathcal{H}_j$ with basis $\{\ket{j,m} |\;
j,m\in\frac{1}{2}\N,\;\; m\ge j\}$
\begin{align*}
K_3\ket{j,m} & = m\ket{j,m}\\
K_\pm\ket{j,m} & = \pm\sqrt{(m\pm j)(m\mp j\pm 1)}\ket{j,m\pm 1}
\end{align*}
while the negative discrete series simply has $m\mapsto -m$.

The Clebsch-Gordon coefficients for the discrete series may be defined
as follows
\begin{equation}\label{CGC-def-O2}
\ket{j\left(j_1 j_2\right),m} = \sum_{m_1,m_2} \left[
\begin{array}{ccc} j_1 & j_2 & j\\ m_1 & m_2 & m \end{array} \right]
\ket{j_1,m_1}\otimes\ket{j_2,m_2}
\end{equation}
with $m = m_1 + m_2$.  An explicit formula for the Clebsch-Gordon
coefficient may be derived via a recursion relation in the manner of
Holman and Biedenharn's approach to the problem (see for instance
\cite{HoBi66} and \cite{HoBi68}). Their formula for the Clebsch-Gordon 
coefficient of coupling in the discrete series consists of the two
solutions $\left[\begin{array}{ccc} j_1 & j_2 & j
\\ m_1 & m_2 & m\end{array}\right]_+$ and 
$\left[\begin{array}{ccc} j_1 & j_2 & j
\\ m_1 & m_2 & m\end{array}\right]_-$ where
\begin{multline}\label{cg}
\left[\begin{array}{ccc} j_1 & j_2 & j
\\ m_1 & m_2 & m\end{array}\right]_+ = 
\delta_{m_1+m_2,m}\\ \times
\sqrt{\frac{\G{m-j+1}\G{m+j}\G{m_1-j_1+1}\G{j_1-j_2+j}\G{j_1+j_2+j-1}}
{\G{m_2-j_2+1}\G{j_2+m_2}\G{m_1+j_1}\G{-j_1+j_2+j}\G{-j_1-j_2+j+1}}}\\
\times\HypT{j_2+m_2}{-m_1+j_1}{m_2-j_2+1}{m_2-j-j_1+1}{m_2+j+j_1}{1}
\end{multline}
and
\begin{equation}\label{cg2}
\left[\begin{array}{ccc} j_1 & j_2 & j
\\ m_1 & m_2 & m\end{array}\right]_- = 
\left[\begin{array}{ccc} j_2 & j_1 & j
\\ -m_2 & -m_1 & -m\end{array}\right]_+
\end{equation}
The particular solution used depends on the case of coupling.

Here a slightly different normalisation to Holman and Beidenharn's
original formula is being used so that the specific formula satisfies
the orthonormality relations in equations \ref{CGC-orth} and
\ref{CGC-orth2},  specifically the usual factor of $\sqrt{2j-1}$ has
been omitted.  Note also that Holman and Beidenharn's formula has the
$j$'s as negative half integers, whereas in equation \ref{cg}
the $j$'s are the more usual positive half integers.

The generalised hypergeometric function\cite{HypGeo} is defined
via
$$
\HypT{a}{b}{c}{d}{e}{z}
= \sum_n \frac{\G{a+n}\G{b+n}\G{c+n}\G{d}\G{e}z^n}
{\G{a}\G{b}\G{c}\G{d+n}\G{e+n}\G{n+1}}
$$
and converges if $-a-b-c+d+e > 0$.


The discrete basis version of the recoupling identity in equation
\ref{racah} may be expressed as
\begin{multline}\label{racah-discrete}
\sum_{m_{12}} 
\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
m_1 & m_2 & m_{12} \end{array} \right]
\left[ \begin{array}{ccc} j_{12} & j_3 & j\\ 
m_{12} & m_3 & m \end{array} \right]\\
= \sum_{j_{23}\;m_{23}} (2j_{23}+1) 
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ j_3 & j & j_{23} 
\end{array}\right\}
\left[ \begin{array}{ccc} j_2 & j_3 & j_{23}\\
m_2 & m_3 & m_{23} \end{array} \right]
\left[ \begin{array}{ccc} j_1 & j_{23} & j\\ 
m_1 & m_{23} & m \end{array} \right]
\end{multline}
where $\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\  m_1 & m_2 &
m_{12} \end{array} \right]$ are the Clebsch-Gordon coefficients for
the coupling of two unitary irreducible representations of $SU(1,1)$. 

The discrete basis version of the orthonormality relations in equation
\ref{CGC-orth} now becomes
\begin{equation}
\sum_{m_1}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ m_1 & m-m_1 & m \end{array} \right]
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ m_1 & m-m_1 & m \end{array} \right]
 = \frac{1}{2j-1} 
\end{equation}
and this relation may be used to bring equation \ref{racah-discrete}
into the following form
\begin{multline} \label{racdef}
\sum_\beta\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
j-j_{23} & \beta & j-j_{23} +\beta \end{array} \right]
\left[ \begin{array}{ccc} j_{12} & j_3 & j\\ 
j-j_{23} +\beta & j_{23}-\beta & j \end{array} \right]
\left[ \begin{array}{ccc} j_2 & j_3 & j_{23}\\ 
\beta & j_{23}-\beta & j_{23} \end{array} \right]\\
= \left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
j_3 & j & j_{23} \end{array}\right\}
\left[ \begin{array}{ccc} j_1 & j_{23} & j\\ 
j-j_{23} & j_{23} & j \end{array} \right]
\end{multline}
where the choice $m_{23} = j_{23}$ has been made.

Depending on the case of coupling one then uses either of
$
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_\pm
$.  From \cite{HoBi68} one must
take
$$
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right] = 
\begin{cases}\renewcommand{\arraystretch}{0.7}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_+ & 
\text{ for }j_1,j_2,j_{12}\in\mathcal{D}^+\\
\renewcommand{\arraystretch}{0.7}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_- & 
\text{\parbox{5cm}{ for $j_1,j\in\mathcal{D}^+$, 
$j_2\in\mathcal{D}^-$\\[-3.5mm] $\,m \ge j_1-j_2$, $m>0$}}\\
\renewcommand{\arraystretch}{0.7}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_+ &
\text{\parbox{5cm}{ for $j_1\in\mathcal{D}^+$,
$j_2,j\in\mathcal{D}^-$\\[-3.5mm] $m \le j_1-j_2$, $m<0$}}\\
\renewcommand{\arraystretch}{0.7}
\left[ \begin{array}{ccc} j_1 & j_2 & j\\ 
m_1 & m_2 & m \end{array} \right]_- & 
\text{ for }j_1,j_2,j_{12}\in\mathcal{D}^- 
\end{cases}
$$

Now consider the representations $j_1$, $j_2$ and $j_3$.  Formally
there are $2^3 = 8$ different combinations of positive and negative
discrete representations, however these come in dual pairs so there
are only four unique possibilities.  It is now a simply matter to
enumerate the possibilities for the remaining discrete series
representations in the Racah coefficent in table \ref{posneg-racah}.

\begin{table}[hbt!]
\begin{center}
\begin{tabular}{ccccccc}
Case & $j_1$ & $j_2$ & $j_3$ & $j_{12}$ & $j_{23}$ & $j$\\
(1) & + & + & + & + & + & +\\
(2) &$-$& + & + & + & + & +\\
(3) &$-$& + & + &$-$& + & +\\
(4) &$-$& + & + &$-$& + &$-$\\
(5) & + & + &$-$& + & + & +\\
(6) & + & + &$-$& + &$-$&$-$\\
(7) & + & + &$-$& + &$-$& +\\
(8) &$-$& + &$-$& + & + & +\\
(9) &$-$& + &$-$& + & + &$-$\\
(10)&$-$& + &$-$&$-$& + &$-$\\
(11)&$-$& + &$-$& + &$-$&$-$\\
(12)&$-$& + &$-$&$-$&$-$&$-$\\
\end{tabular}
\end{center}
\caption{The possible unique distributions of positive and negative discrete 
representations in the Racah coefficient\label{posneg-racah}}
\end{table}

Consider the Clebsch-Gordon coefficient on the right hand side of
equation \ref{racdef}.  One has
$$
\left[\begin{array}{ccc}
j_1 & j_{23} & j\\
m_1 & j_{23} & j
\end{array}\right] = 
\begin{cases}
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & m_1 & j_{23}+m_1
\end{array}\right]_+ & \text{for cases 1 and 5}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
-j_{23} & -m_1 & -j_{23}-m_1
\end{array}\right]_- & \text{for cases 11 and 12}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & -m_1 & j_{23}-m_1
\end{array}\right]_- & \text{for cases 2, 3 and 8}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & -m_1 & j_{23}-m_1
\end{array}\right]_+ & \text{for cases 4, 9 and 10}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_1 & j_{23} & j\\
m_1 & -j_{23} & m_1-j_{23}
\end{array}\right]_+ & \text{for case 6}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_1 & j_{23} & j\\
m_1 & -j_{23} & m_1-j_{23}
\end{array}\right]_- & \text{for case 7}\\
\end{cases}
$$

Now note that by equation \ref{cg2} there are only three unique
evaluations to be made since 
$$
\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & m_1 & j_{23}+m_1
\end{array}\right]_+ = \left[\begin{array}{ccc}
j_{23} & j_1 & j\\
-j_{23} & -m_1 & -j_{23}-m_1
\end{array}\right]_-
$$
and cases 1, 5, 11 and 12 are equivalent here, also
$$\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & -m_1 & j_{23}-m_1
\end{array}\right]_- = \left[\begin{array}{ccc}
j_1 & j_{23} & j\\
m_1 & -j_{23} & m_1-j_{23}
\end{array}\right]_+
$$
so that cases 2, 3, 6 and 8 have the same Clebsch-Gordon coefficient,
and
$$
\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & -m_1 & j_{23}-m_1
\end{array}\right]_+ = \left[\begin{array}{ccc}
j_1 & j_{23} & j\\
m_1 & -j_{23} & m_1-j_{23}
\end{array}\right]_-
$$
allowing cases 4, 7, 9 and 10 to be treated together.

For these last for cases the value of $m_1$ will be fixed as $m_1 =
j_1$, while for the first four cases, 1, 5, 11 and 12, take $m_1 =
j-j_{23}$.  The remaining four cases have $m_1 = j_{23}-j$.

In the following any constant phase may, and will, be discarded since
the phase of the Racah coefficient is arbitrary.  Hence all the
equalities are modulo a phase.  In addition the $\Gamma$ functions may
need to be understood in terms of their analytic continuations via
lemma \ref{lem2}, depending on the specifics of the cases of coupling.

By direct evaluation one may show, for cases 1, 2, 3, 5, 6, 8, 11 and
12,
\begin{multline}
\left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & j-j_{23} & j
\end{array}\right]_+ = \left[\begin{array}{ccc}
j_1 & j_{23} & j\\
-j+j_{23} & -j_{23} & -j
\end{array}\right]_+\\
 = \sqrt{\frac{\G{j_{23}+j-j_1}\G{j+j_1+j_{23}-1}}{\G{2j}\G{2j_{23}}}}
\end{multline}

The result for $\left[\begin{array}{ccc}
j_1 & j_{23} & j\\
j-j_{23} & j_{23} & j
\end{array}\right]_+$ follows immediately from equation \ref{cg} and
the fact that 
$$
\sum_{n\in\Z}
\frac{A\left(n\right)}{\G{1-r+n}\G{1+r-n}} = A\left(r\right)
$$
for $r\in\Z$

The other evaluation requires the Gauss summatation formula (lemma
\ref{lem3}) to evaluate the sum in the hypergeometric series and
repeated applications of lemma \ref{lem2} to bring it into the same
form.

For the remaining cases, 4,7,9 and 10, one has
\begin{multline}
\left[\begin{array}{ccc}
j_1 & j_{23} & j\\
j_1 & -j_{23} & j_1-j_{23}
\end{array}\right]_- = \left[\begin{array}{ccc}
j_{23} & j_1 & j\\
j_{23} & -j_1 & j_{23}-j_1
\end{array}\right]_- \\
 = \sqrt{\frac{\G{j_{23}-j+j_1}\G{j+j_1+j_{23}-1}}{\G{2j}\G{2j_{23}}}}
\end{multline}
again by a direct evaluation and repeated use of lemma \ref{lem2}.


Similarly consider the Clebsch-Gordon coefficient that determines the
coupling of $j_2$ and $j_3$. Once the cases that are dual to each
other have been combined one has again three cases
\begin{equation}
\left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
\beta & j_{23}-\beta & j_{23}
\end{array}\right] = 
\begin{cases}
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
\beta & j_{23}-\beta & j_{23}
\end{array}\right]_+ & \text{for cases 1, 2, 3 and 4}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
\beta & -j_{23}-\beta & -j_{23}
\end{array}\right]_+ & \text{for cases 6, 7, 11 and 12}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
\beta & j_{23}-\beta & j_{23}
\end{array}\right]_- & \text{for cases 5, 8, 9 and 10}
\end{cases}
\end{equation}

Again, a direct evaluation in the same manner as the previous case
shows that two of these are equal. Thus for cases 1, 2, 3, 4, 5, 8, 9,
and 10 it may be may be evaluated as
\begin{multline}
\left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
\beta & j_{23}-\beta & j_{23}
\end{array}\right]_+ = \left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
\beta & j_{23}-\beta & j_{23}
\end{array}\right]_-
\\ = 
\frac{\left(-1\right)^b\Delta\left(j_2 j_3 j_{12}\right)}
{\sqrt{\G{2j_{23}}\G{\beta+j_2}\G{j_{23}-j_3-\beta+1}}}\\
\times\frac{1}{\sqrt{\G{\beta-j_2+1}\G{j_3+j_{23}-\beta}}}
\end{multline}
where
\begin{multline*}
\Delta\left(j_1 j_2 j_{12}\right) = \sqrt{
\G{j_1+j_2+j-1}\G{-j_1+j_2+j}}\\
\times\sqrt{\G{j_1-j_2+j}\G{-j_1-j_2+j+1}}
\end{multline*}

The third, covering cases 6, 7, 11 and 12, may be evaluated as
\begin{multline}
\left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
\beta & -j_{23}-\beta & -j_{23}
\end{array}\right]_+ = \left[\begin{array}{ccc}
j_2 & j_3 & j_{23}\\
-\beta & j_{23}+\beta & j_{23}
\end{array}\right]_+\\ = 
\frac{\left(-1\right)^b\Delta\left(j_2 j_3 j_{12}\right)}
{\sqrt{\G{2j_{23}}\G{\beta+j_2}\G{j_{23}-j_3+\beta+1}}}\\
\times\frac{1}{\sqrt{\G{-\beta-j_2+1}\G{j_3+j_{23}+\beta}}}
\end{multline}

Next, consider the Clebsch-Gordon coefficient 
$\left[\begin{array}{ccc}
j_{12} & j_3 & j\\
j-j_{23}+\beta & j_{23}-\beta & j
\end{array}\right]$. After combining cases related by equation
\ref{cg2} and making sure to preserve the assignments made to $m_1$
\begin{multline}
\left[\begin{array}{ccc}
j_{12} & j_3 & j\\
j-j_{23}+\beta & j_{23}-\beta & j
\end{array}\right] =\\ 
\begin{cases}
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_3 & j_{12} & j\\
j_{23}-\beta & j-j_{23}+\beta & j
\end{array}\right]_+ & \text{for cases 1 and 2}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_3 & j_{12} & j\\
j_{23} - \beta& \beta-j_{23}+j & j
\end{array}\right]_- & \text{for cases 3, 5 and 8}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_3 & j_{12} & j\\
j_{23}-\beta & -j_1 +\beta & j_{23}-j_1
\end{array}\right]_+ & \text{for case 4}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_{12} & j_3 & j\\
 -j_1 +\beta & j_{23}-\beta & j_{23}-j_1
\end{array}\right]_+ & \text{for case 9}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_3 & j_{12} & j\\
j_{23}-\beta & -j_1 +\beta & j_{23}-j_1
\end{array}\right]_- & \text{for case 10}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_{12} & j_3 & j\\
-j+j_{23}+\beta & -j_{23}-\beta & -j
\end{array}\right]_+ & \text{for cases 6, 11 and 12}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_{12} & j_3 & j\\
j_1+\beta & -j_{23} -\beta & -j_{23}+j_1
\end{array}\right]_- & \text{for case 7}
\end{cases}
\end{multline}

Direct evaluation as in the previous two cases yields the following
explicit formulae for cases 1, 2, 3, 5 and 8
\begin{multline}
\left[\begin{array}{ccc}
j_3 & j_{12} & j\\
j_{23}-\beta & j-j_{23}+\beta & j
\end{array}\right]_+ = \left[\begin{array}{ccc}
j_3 & j_{12} & j\\
j_{23}-\beta & j-j_{23}+\beta & j
\end{array}\right]_-\\
= \frac{\left(-1\right)^\beta\Delta\left(j_3j_{12}j\right)}
{\sqrt{\G{2j}\G{j-j_{23}-j_{12}+\beta+1}\G{j_{12}+j-j_{23}+\beta}}}\\
\times\frac{1}{\sqrt{\G{j_{23}-\beta-j_3+1}\G{j_3+j_{23}-\beta}}}
\end{multline}

and, for cases 6, 11 and 12,

\begin{multline}
\left[\begin{array}{ccc}
j_{12} & j_3 & j\\
-j+j_{23}+\beta & -j_{23}-\beta & -j
\end{array}\right]_+ \\
= \frac{\left(-1\right)^\beta\Delta\left(j_3j_{12}j\right)}
{\sqrt{\G{2j}\G{j-j_{23}-j_{12}-\beta+1}\G{j_{12}+j-j_{23}-\beta}}}\\
\times\frac{1}{\sqrt{\G{j_{23}+\beta-j_3+1}\G{j_3+j_{23}+\beta}}}
\end{multline}

The remaining four cases remain as sums and one has, for cases 4, 9
and 10,
\begin{multline}
\left[\begin{array}{ccc}
j_3 & j_{12} & j\\
j_{23}-\beta & \beta-j_1 & j_{23}-j_1
\end{array}\right]_- = \frac{\Delta\left(j_3 j_{12}j\right)}
{\G{j_3+j-j_{12}}\G{j-j_{12}-j_3+1}}\\ \times
\sqrt{\frac{\G{j_1-j_{23}-j+1}\G{j_1-j_{23}+j}\G{j_1-j_{12}+1-\beta}}
{\G{1-j_3-j_{23}+\beta}\G{j_3-j_{23}+\beta}\G{j_1+j_2-\beta}}}\\ \times
\sum_n\frac{\left(-1\right)^n\G{j_{12}-j_1-\beta+n}\G{-j_1-j_{12}-\beta+1+n}}
{\G{-j_1-\beta-j+j_3+1+n}\G{-j_1-\beta+j+j_3+n}}\\ \times
\frac{1}{\G{1+j_{23}-j_3+\beta-n}\G{n+1}}
\end{multline}
and for case 7,
\begin{multline}
\left[\begin{array}{ccc}
j_{12} & j_3 & j\\
j_1 + \beta & -j_{23}-\beta & j_1-j_{23}
\end{array}\right]_- = \frac{\Delta\left(j_3 j_{12} j\right)}
{\G{j+j_{12}-j_3}\G{j-j_{12}-j_3+1}}\\ \times
\sqrt{\frac{\G{j_{23}-j_1-j+1}\G{j_{23}-j_1+j}\G{j_{23}+\beta-j_3+1}}
{\G{-j_1-j_{12}-\beta+1}\G{j_{12}-j_1-\beta}\G{j_{23}+\beta+j_3}}}\\
\times\sum_n\frac{\left(-1\right)^n\G{j_{12}-j_1-\beta+n}
\G{-j_1-\beta-j_{12}+1+n}}{\G{-j_1-\beta-j+j_3+1+n}\G{-j_1-\beta+j+j_3+n}}
\\ \times
\frac{1}{\G{1+j_{23}+\beta-j_3-n}\G{n+1}}
\end{multline}

The final Clebsch-Gordon coefficient to consider is $
\left[\begin{array}{ccc}
j_1 & j_2 & j_{12}\\ j-j_{23} & \beta & j-j_{23}+\beta
\end{array}\right]$.   After cases of coupling that are equivalent by
equation \ref{cg2} are combined one has
\begin{multline}
\left[\begin{array}{ccc}
j_1 & j_2 & j_{12}\\ j-j_{23} & \beta & j-j_{23}+\beta
\end{array}\right]\\ = 
\begin{cases}
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & j-j_{23} & j-j_{23}+\beta
\end{array}\right]_+ & \text{for cases 1, 5 and 12}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & j_{23}-j & j_{23}-j+\beta
\end{array}\right]_+ & \text{for cases 3 and 6}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & j-j_{23} & j-j_{23}+\beta
\end{array}\right]_- & \text{for cases 2, 8 and 11}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & j_1 & j_1+\beta
\end{array}\right]_+ & \text{for case 7}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & -j_{1} & -j_{1}+\beta
\end{array}\right]_- & \text{for case 9}\\
\renewcommand{\arraystretch}{0.7}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & -j_{1} & -j_{1}+\beta
\end{array}\right]_+ & \text{for cases 4 and 10}\\
\end{cases}
\end{multline}

As before a direct evaluation of these Clebsch-Gordon coefficients
yields, for cases 4, 9 and 10,
\begin{multline}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & -j_{1} & -j_{1}+\beta
\end{array}\right]_+ = \left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & -j_{1} & -j_{1}+\beta
\end{array}\right]_-\\
= \frac{\Delta\left(j_1 j_2 j_{12}\right)}
{\sqrt{\G{2j_1}\G{j_{12}-j_1-j_2+1}\G{-j_1+j_2+j_{12}}}}\\
\times\sqrt{\frac{\G{\beta-j_1-j_2+1}\G{\beta-j_1+j_{12}}}
{\G{\beta-j_2+1}\G{\beta+j_2}}}
\end{multline}

For case 7,
\begin{multline}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & j_1 & j_1+\beta
\end{array}\right]_+ =  \frac{\Delta\left(j_1 j_2 j_{12}\right)}
{\sqrt{\G{2j_1}\G{j_{12}-j_1-j_2+1}\G{-j_1+j_2+j_{12}}}}\\
\times\sqrt{\frac{\G{\beta-j_2+1}\G{\beta+j_{2}}}
{\G{\beta+j_1-j_2+1}\G{\beta+j_1+j_{12}}}}
\end{multline}

The remaining cases are only expressible as sums. One has, for cases
2, 8 and 11,
\begin{multline}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & j-j_{23} & \beta+j-j_{23}
\end{array}\right]_+ = \frac{\Delta\left(j_1 j_2 j_{12}\right)}
{\sqrt{\G{j_1+j_{12}-j_2}\G{j_{12}-j_1-j_2+1}}}\\ \times
\sqrt{\frac{\G{\beta+j-j_{23}-j_{12}+1}
\G{-j_{23}+\beta+j+j_{12}}\G{\beta-j_2+1}}
{\G{\beta+j_2}\G{j_{23}-j_1-j+1}\G{j_1-j_{23}+j}}}\\ \times
\sum_n\frac{\left(-1\right)^n\G{j_1-j_{23}+j+n}\G{j-j_{23}-j_1+1+n}}
{\G{j-j_{23}-j_{12}+j_2+1+n}\G{j-j_{23}+j_{12}+j_2+n}
\G{1+\beta-j_2-n}\G{n+1}}
\end{multline}

For cases 1, 5 and 12,
\begin{multline}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & -j+j_{23} & \beta-j+j_{23}
\end{array}\right]_+ = \frac{\Delta\left(j_1 j_2 j_{12}\right)}
{\sqrt{\G{j_1+j_{12}-j_2}\G{j_{12}-j_1-j_2+1}}}\\ \times
\sqrt{\frac{\G{\beta+j_{23}+j-j_{12}+1}
\G{j_{23}+\beta-j+j_{12}}\G{\beta-j_2+1}}
{\G{\beta+j_2}\G{j_{23}+j_1-j}\G{-j_1+j_{23}-j+1}}}\\ \times
\sum_n\frac{\left(-1\right)^n\G{j_1+j_{23}-j+n}\G{j_{23}-j-j_1+1+n}}
{\G{j_{23}-j-j_{12}+j_2+1+n}\G{j_{23}-j+j_{12}+j_2+n}
\G{1+\beta-j_2-n}\G{n+1}}
\end{multline}

and finally for cases 3 and 6
\begin{multline}
\left[\begin{array}{ccc}
j_2 & j_1 & j_{12}\\ \beta & j-j_{23} & \beta+j-j_{23}
\end{array}\right]_- = \frac{\Delta\left(j_1 j_2 j_{12}\right)}
{\sqrt{\G{j_1+j_{12}-j_2}\G{j_{12}-j_1-j_2+1}}}\\ \times
\sqrt{\frac{\G{j_{23}-\beta-j-j_{12}+1}
\G{j_{23}-j-\beta+j_{12}}\G{j_{23}-j_1-j+1}}
{\G{1-\beta-j_2}\G{j_{23}+j_1-j}\G{-\beta+j_2}}}\\ \times
\sum_n\frac{\left(-1\right)^n\G{-\beta+j_2+n}\G{-\beta-j_2+1+r}}
{\G{j_1-j_{12}-\beta+1+n}\G{j_1+j_{12}-\beta+n}
\G{1-j_1+j_{23}-j-n}\G{n+1}}
\end{multline}

It now remains to calculate the Racah cofficient for the twelve cases
given in table \ref{posneg-racah}.  Let the Racah coefficient for each
of the twelve cases of coupling be denoted by a subscript $N$ for
$N=1\dots 12$.

First note that cases 1 and 5 may be grouped together since the
Clebsch-Gordon coefficients have been shown to have exactly the same
form for these two cases.  Thus the resulting Racah coefficient
consists of one equation that may be analytically continued, using
lemma \ref{lem3}, to the respective domains of definition and its
value is preserved by this.  In a similar way cases 4, 9 and 10 may be
combined, as may cases 2 and 8.

Explicitly the calculation for cases 1 proceeds from a substitution of
equation
\ref{cg} into \ref{racdef}, which gives the following
\begin{equation} \label{rac2}
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ j_3 & j & j_{23} \end{array} 
\right\}_1 = \Delta\left(j_2 j_3 j_{23}\right)
\Delta\left(j_{12}j_3 j\right)\Delta\left(j_1 j_{23} j\right)
\Delta\left(j_1 j_2 j_{12}\right)\,\mathcal{I}
\end{equation}
where
\begin{multline*}
\mathcal{I} =\sum_{t\,\beta}\left(-1\right)^{j-j_{23}-j_{12}-j_2+t+2\beta}
\frac{\G{\beta+j_2+t}\G{\beta-j_2+1+t}}
{\G{j_{23}-\beta-j_3+1}\G{j_3+j_{23}-\beta}\G{\beta-j_2+1}}\\
\times\frac{1}{\G{j_1+j-j_{23}}\G{\beta-j_{12}+j_1+1+t}\G{j_1+j_{12}+\beta+t}
\G{\beta+j_2}\G{t+1}}\\
\times\frac{1}{\G{1-j_1+j-j_{23}-t}\G{j_2-j_1+j_{12}}\G{j_{12}-j_1-j_2+1}
\G{j+j_{23}-j_1}}\\ \times\frac{1}{\G{j_1+j_{23}+j-1}}
\end{multline*}

$\mathcal{I}$ may be reduced to a single summation as follows.
Introduce a new summation using lemma \ref{lem1} with $a =
\beta-j_2+t$, $b = \beta-j_{12}+j_1+t$ and $c = \beta+j_1+j_{12}+t-1$,
then $\mathcal{I}$ may be written (after an application of equation
\ref{an-cont})
\begin{multline*}
\mathcal{I} = \sum_{\beta\,u\,t}\left(-1\right)^{2\beta+j-j_2-j_{12}-j_{23}}
\frac{\G{\beta+j_2+t}\G{j_1-j+j_{23}+t}\G{-j_1-j_2-j_{12}+2}}
{\G{j_{23}-\beta-j_3+1}\G{j_3+j_{23}-\beta}\G{\beta-j_2+1}\G{\beta+j_2}}\\
\times\frac{1}{\G{j_1+j-j_{23}}\G{t+1}\G{j_2-j_1+j_{12}}\G{j+j_{23}-j_1}
\G{j_1+j+j_{23}-1}}\\
\times\frac{1}{\G{j_{12}-j_2-j_1-u+1}\G{2-j_1-j_2-j_{12}-u}
\G{2j_1+\beta+j_2+t+u}\G{u+1}}\\
\times\frac{1}{\G{j_1+j_{23}-j}\G{j-j_1-j_{23}+1}}
\end{multline*}

The sum over $t$ is simply a hypergeometric function at $z=1$.  This
may be summed by Gauss' theorem, as in lemma \ref{lem3} with $a =
\beta+j_2$, $b = j_1+j_{23}-j$ and $c = \beta +2j_1+j_2+u$.  The
remaining sums may be written
\begin{multline*}
\mathcal{I} =
\sum_{\beta\,u}\left(-1\right)^{2\beta-j_2+j-j_{23}-j_{12}}
\frac{\G{2-j_2-j_1-j_{12}}\G{j+j_1-j_{23}+u}}
{\G{j_{23}-j_3-\beta+1}\G{j_3+j_{23}-\beta}\G{\beta-j_2+1}}\\
\times\frac{1}{\G{j+j_1-j_{23}}\G{j_2-j_1+j_{12}}\G{j_{23}+j-j_1}
\G{j_1+j_{23}+j-1}}\\\times\frac{1}
{\G{j_{12}-j_1-j_2-u+1}\G{2-j_1-j_2-j_{12}-u}\G{u+1}\G{j-j_1-j_{23}+1}}
\\ \times\frac{1}{\G{2j_1+u}\G{j_1+j_2+j-j_{23}+u+\beta}}
\end{multline*}

Now set $\beta = z+j_2$, with $z$ now guaranteed to be an integer.
The sum over $z$, after two applications of equation \ref{an-cont},
may be again be recognised as a hypergeometric function which is
summable by Gauss' theorem, using lemma \ref{lem3} with $a =
j_2+j_3-j_{23}$, $b = 1+j_2-j_3-j_{23}$ and $c = 2j_2+j_1+u+j-j_{23}$.

The final sum over $u$ is a generalised hypergeometric function of
type ${ }_4F_3$ and the sum $\mathcal{I}$ may be written

\begin{multline*}
\mathcal{I} = \left(-1\right)^{j_2+j-j_{23}-j_{12}}
\frac{1}{\G{j_{12}-j_1+j_2}\G{j+j_{23}-j_1}\G{j-j_1-j_{23}+1}}\\
\times\frac{1}{\G{j_{23}-j_2-j_3+1}\G{j_{23}+j_3-j_2}\G{j_{12}-j_1-j_2+1}}\\
\times\frac{1}{\G{2j_1}\G{j_1+j_2-j_3}\G{j_1+j_2-1+j_3}}\\
\times\HypF{j_1+j-j_{23}}{j_1+j+j_{23}-1}{j_1+j_2-j_{12}}
{j_1+j_2+j_{12}-1}{2j_1}{j_1+j_2+j-j_3}{j_1+j_2+j_3+j-1}{1}
\end{multline*}

where the generalised hypergeometric function\cite{HypGeo} is defined as
\begin{multline*}
\HypF{a}{b}{c}{d}{e}{f}{g}{z} = \\
\sum_n\frac{\G{a+n}\G{b+n}\G{c+n}\G{d+n}\G{e}\G{f}\G{g}}
{\G{a}\G{b}\G{c}\G{d}\G{e+n}\G{f+n}\G{g+n}\G{n+1}}z^n
\end{multline*}

subsitituting this back into equation \ref{rac2} the final result is
gained
\begin{multline}\label{Racah-Su11-hyper}
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ j_3 & j & j_{23} \end{array} 
\right\}_1 = \frac{\left(-1\right)^{j_2+j-j_{23}-j_{12}}
\Delta\left(j_2 j_3 j_{23}\right)
\Delta\left(j_{12}j_3 j\right)\Delta\left(j_1 j_{23} j\right)}
{\G{j_{12}-j_1+j_2}\G{j+j_{23}-j_1}\G{j-j_1-j_{23}+1}}\\
\times\frac{\Delta\left(j_1 j_2 j_{12}\right)}
{\G{j_{23}-j_2-j_3+1}\G{j_{23}+j_3-j_2}\G{j_{12}-j_1-j_2+1}}\\
\times\frac{1}{\G{2j_1}\G{j_1+j_2-j_3}\G{j_1+j_2-1+j_3}}\\
\times\HypF{j_1+j-j_{23}}{j_1+j+j_{23}-1}{j_1+j_2-j_{12}}
{j_1+j_2+j_{12}-1}{2j_1}{j_1+j_2+j-j_3}{j_1+j_2+j_3+j-1}{1}
\end{multline}

In a similar way one may derive the formula for case 5 as
\begin{multline}
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}
\\ j_3 & j & j_{23} \end{array} \right\}_5 
= \frac{\left(-1\right)^{2j_3-2j_{23}-1}
\Delta\left(j_1 j_2 j_{12}\right)
\Delta\left(j_3 j_{23}j_2\right)}
{\G{j_2+j_{23}-j_3}\G{j_{12}-j_3-j+1}\G{j_2+j_3+j_{23}-1}}\\
\times\frac{\Delta\left(j_{23} j_1 j\right)
\Delta\left(j j_3 j_{12}\right)\G{2j_{23}-1}}
{\G{j_1-j_2+j_{12}}\G{j_{12}-j_1-j_2+1}
\G{j+j_{23}-j_1}\G{j_3+j_{12}-j}}\\ 
\times\frac{1}{\G{j_1+j_{23}+j-1}
\G{j+j_2-j_{12}-j_{23}+1}\G{j-j_{23}+j_{12}+j_2}}\\ 
\times
\HypF{j+j_1-j_{23}}{j-j_{23}-j_1+1}{j_2+j_3-j_{23}}{j_2-j_3-j_{23}+1}
{j+j_2-j_{12}-j_{23}+1}{j+j_2+j_{12}-j_{23}}{2-2j_{23}}{1}
\end{multline}

From the explicit case by case calculations of the Clebsch-Gordon
coefficients it is expected that these two Racah coefficients are
analytic continuations of each other, with each coefficient valid in a
domain where the $j$'s satisfy two different regimes of anti-triangle
inequalities.  To see this note that
\begin{multline}
\frac{\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}
\\ j_3 & j & j_{23} \end{array} \right\}_1 }
{\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}
\\ j_3 & j & j_{23} \end{array} \right\}_5 }=
\left(-1\right)^{j_2+j-j_{12}+j_{23}+2j_3} 
\sqrt{\frac{\G{j-j_3-j_{12}+1}\G{j_3-j_{12}+j}}
{\G{j_{23}-j-j_3+1}\G{j_3-j_2+j_{23}}}}\\ \times
\sqrt{\frac{\G{j_{12}-j_3-j+1}\G{j_3+j_{12}-j}}
{\G{j_2+j_3-j_{23}}\G{j_2-j_3-j_{23}+1}}} 
= \left(-1\right)^{j_2+j-j_{12}+j_{23}+2j_3} 
\end{multline}
with the final equality from suitable applications of equation
\ref{an-cont}.

The strategy for evaluating the remaining cases is similar and the
details will be omitted in favour of the end realisation of the Racah
coefficient in terms of a generalised ${ }_4F_3$ hypergeometric
function which covers the relevant cases using the analytic
continuations of lemma \ref{lem2} as necessary.

Case 4 
\begin{multline}
\left\{ \begin{array}{ccc} j_1 & j_2 & j_{12}
\\ j_3 & j & j_{23} \end{array} \right\}_4
=\frac{\left(-1\right)^{j_2+j_3+j-j_1-\frac{1}{2}}
\Delta\left(j_2j_{12}j_1\right)\Delta\left(j_2j_3j_{23}\right)
\Delta\left(j_{23}jj_1\right)}{\G{j_3-j_2+j_{23}}\G{j+j_{12}-j_3}
\G{j_1-j_2+j_{12}}}\\ \times
\frac{\Delta\left(j_3 jj_{12}\right)
\G{j_2-j_1+j_{12}}\G{j_2+j_3-j_{23}}}
{\G{j_1+j+j_{23}-1}\G{j_1-j+j_{23}}\G{j_1-j_{23}-j+1}
\G{j_{12}-j_3-j+1}}\\ \times
\frac{1}{\G{j_2+j_3-j_1-j+1}\G{j_2+j_3-j_1+j}\G{2j_2}
\G{j_1+j-j_{23}}}\\
\HypF{j_2-j1+j_{12}}{j_2-j_1-j_{12}+1}{j_3+j_{23}+j_2-1}
{j_2+j_3-j_{23}}{j_2+j_3-j_1-j+1}{j_2+j_3+j-j_1}{2j_2}{1}
\end{multline}

Case 9



There are two symmetries one may apply to equation \ref{racdef} in
order to generate the twelve different cases of coupling.

Firstly, consider the symmetry where $j_{12}$ is swapped with $j_{23}$
and $j_1$ is swapped with $j_3$, applied to equation
\ref{racdef}.  One now has
\begin{multline}
\sum_\beta\left[ \begin{array}{ccc} j_3 & j_2 & j_{23}\\ 
j-j_{12} & \beta & j-j_{12} +\beta \end{array} \right]
\left[ \begin{array}{ccc} j_{23} & j_1 & j\\ 
j-j_{12} +\beta & j_{12}-\beta & j \end{array} \right]
\left[ \begin{array}{ccc} j_2 & j_1 & j_{12}\\ 
\beta & j_{12}-\beta & j_{12} \end{array} \right]\\
= \left\{ \begin{array}{ccc} j_3 & j_2 & j_{23}\\ 
j_1 & j & j_{12} \end{array}\right\}
\left[ \begin{array}{ccc} j_3 & j_{12} & j\\ 
j-j_{12} & j_{12} & j \end{array} \right]
\end{multline}

This equation is the defining relation for a Racah coefficient with a
potentially different distribution of positive and negative discrete
series.  In particular it is easy to see from table \ref{posneg-racah}
that it causes the following exchanges: case 2 is swapped with case 5,
case 3 is swapped with case 7, case 4 is swapped with case 6 and case
10 is swapped with case 11.  The remainder are left invariant.

The second symmetry is where $j_1$ is swapped with $j_2$ and $j_3$ is
swapped with $j$.  Applying this to the defining relation for the
Racah coefficient, written as the recoupling relation as in equation
\ref{racah-discrete}, one finds the following transformations occur to
the Clebsch-Gordon coefficients (again a particular choice of basis
elements has been made):
\begin{multline*}
\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
j - m_{23} & m_{12} - j + m_{23} & m_{12}
\end{array} \right] 
\longmapsto\left[ \begin{array}{ccc} j_2 & j_1 & j_{12}\\ 
j_3 - m_{23} & m_{12} - j_3 + m_{23} & m_{12}
\end{array} \right] \\ =  
\left[ \begin{array}{ccc} j_1 & j_2 & j_{12}\\ 
m_{12} - j_3 + m_{23} & j_3 - m_{23} & m_{12}
\end{array} \right]
\end{multline*}
\begin{multline*}
\left[ \begin{array}{ccc} j_2 & j_3 & j_{23}\\ 
m_{12} - j + m_{23} & j-m_{12} & m_{23} 
\end{array} \right] 
\longmapsto\left[ \begin{array}{ccc} j_1 & j & j_{23}\\ 
m_{12} - j_3 +m_{23} & j_3 - m_{12} & m_{23} 
\end{array} \right]\\ = 
\left[ \begin{array}{ccc} j_1 & j_{23} & j\\ 
m_{12} - j_3 +m_{23} & -m_{23}  & - j_3 + m_{12}  
\end{array} \right]
\end{multline*}
$$
\left[ \begin{array}{ccc} j_1 & j_{23} & j\\ 
j - m_{23} & m_{23} & j \end{array} \right] 
\longmapsto\left[ \begin{array}{ccc} j_2 & j_{23} & j_{3}\\ 
j_3 - m_{23} & m_{23} & j_3 \end{array} \right] = 
\left[ \begin{array}{ccc} j_2 & j_3 & j_{23}\\ 
j_3 - m_{23} & -j_3 & -m_{23} \end{array} \right]
$$
$$
\left[ \begin{array}{ccc} j_{12} & j_3 & j\\ 
m_{12} & - m_{12} + j & j \end{array} \right] 
\longmapsto\left[ \begin{array}{ccc} j_{12} & j & j_3\\ 
m_{12} & - m_{12} + j_3 & j_3 \end{array} \right]\\  = 
\left[ \begin{array}{ccc} j_{12} & j_3 & j\\ 
m_{12} &  -j_3 & m_{12} - j_3 \end{array} \right]
$$

The final equalities will not be justified here since they, and
symmetries like them, are the subject of section \ref{inv}, although
it is possible to verify them directly for the cases where all
representations are in the discrete series from the defintions of the
Clebsch-Gordon coefficients in equations \ref{cg} and \ref{cg2}.  In
essence they are the \su{1,1} analogue of the well known permutation
symmetries for the \su{2} Clebsch-Gordon coefficient\cite{AngMom}.

The above symmetry has the property that it induces the following
exchanges among the different cases of coupling in table
\ref{posneg-racah}: case 1 is swapped with case 6, case 2 is swapped
with case 3, case 4 is swapped with case 8, case 5 is swapped with
case 7, case 9 is swapped with case 10 and case 11 is swapped with
case 12.

It is now possible to generate all the twelve different cases of
coupling in table \ref{posneg-racah} using the formulae in equations
\ref{Racah-Su11-hyper} and \ref{4-9-10}.  These two equations cover
five cases as they stand, then the above two symmetries may be used to
extend them to formulae covering the full twelve cases.


